Learning to Estimate Shapley Values with Vision Transformers

Transformers have become a default architecture in computer vision, but understanding what drives their predictions remains a challenging problem. Current explanation approaches rely on attention values or input gradients, but these provide a limited view of a model's dependencies. Shapley values offer a theoretically sound alternative, but their computational cost makes them impractical for large, high-dimensional models. In this work, we aim to make Shapley values practical for vision transformers (ViTs). To do so, we first leverage an attention masking approach to evaluate ViTs with partial information, and we then develop a procedure to generate Shapley value explanations via a separate, learned explainer model. Our experiments compare Shapley values to many baseline methods (e.g., attention rollout, GradCAM, LRP), and we find that our approach provides more accurate explanations than existing methods for ViTs.

==> ViT Shapley (ICLR 2023)/figures/ablations.tex <==
\begin{table}[h]
\centering
\caption{
Ablation experiments for ViT Shapley explainer architecture on the ImageNette dataset, with and without fine-tuning.
} \label{tab:ablations}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{scriptsize}
% {\tablesize
    % \begin{tabular}{cccccc}
    % \toprule
    % Configuration & Extra attention block & Frozen backbone & Removal method & Val loss & Test loss \\
    % \midrule
    % % \#1 & False & False & Masking (fine-tuned) & 4.351 \\
    % % \#2 & False & True & Masking (fine-tuned) & 4.351 \\
    % % \#3 & True & False & Masking (fine-tuned) & \textbf{4.318} \\
    % % \#4 & True & True & Masking (fine-tuned) & 4.339 \\
    % A & False & True & Masking (fine-tuned) & 4.332 & 4.351 \\
    % B & False & False & Masking (fine-tuned) & 4.331 & 4.351 \\
    % C & True & True & Masking (fine-tuned) & 4.319 & 4.339 \\
    % D & True & False & Masking (fine-tuned) & \textbf{4.309} & \textbf{4.318} \\
    % % \#5 & True & False & Mask token (fine-tuned) & 4.388 \\
    % \midrule
    % \multicolumn{3}{c}{ViT trained from scratch} & Masking (fine-tuned) & 4.331 & 4.341 \\
    % \midrule
    % \multicolumn{3}{c}{U-Net trained from scratch} & Masking (fine-tuned) & 4.332 & 4.338 \\
    % \bottomrule
    % \end{tabular}
    \begin{tabular}{ccccc}
    \toprule
    Fine-tuning config. & Extra attention block & Frozen backbone & Val loss & Test loss \\
    \midrule
    A & False & True & 4.332 & 4.351 \\
    B & False & False & 4.331 & 4.351 \\
    C & True & True & 4.319 & 4.339 \\
    D & True & False & \textbf{4.309} & \textbf{4.318} \\
    \midrule
    \multicolumn{3}{c}{ViT trained from scratch} & 4.331 & 4.341 \\
    \midrule
    \multicolumn{3}{c}{U-Net trained from scratch} & 4.332 & 4.338 \\
    \bottomrule
    \end{tabular}
% }
% \end{scriptsize}
\end{small}
\end{center}
\end{table}


==> ViT Shapley (ICLR 2023)/figures/insertion_curves_imagenette.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{images/insertion_curves_imagenette.pdf}
    \caption{
    ImageNette average insertion/deletion curves. \textbf{Top:} the mean prediction probability for the target class as features are inserted or deleted in order of most to least important.
    \textbf{Bottom:} the mean prediction probability, averaged across all non-target classes.
    }
    \label{fig:insertion_curves_imagenette}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/insertion_curves_mura.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{images/insertion_curves_mura.pdf}
    \caption{
    MURA average insertion/deletion curves. The mean prediction probability for the target class is plotted as features are inserted or deleted in order of most to least important.
    }
    \label{fig:insertion_curves_mura}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/insertion_curves_pet.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{images/insertion_curves_pet.pdf}
    \caption{
    Pets average insertion/deletion curves.
    \textbf{Top:} the mean prediction probability for the target class as features are inserted or deleted in order of most to least important.
    \textbf{Bottom:} the mean prediction probability, averaged across all non-target classes.
    }
    \label{fig:insertion_curves_pet}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/kernelshap.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/kernelshap.pdf}
    \caption{
    ViT Shapley vs. KernelSHAP comparison (ImageNette). 
    }
    \label{fig:kernelshap}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/kernelshap_error.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/kernelshap_error.pdf}
    \caption{
    Comparing the quality of Shapley value estimates obtained by ViT Shapley and KernelSHAP. The shaded areas represent 95\% confidence intervals.
    }
    \label{fig:kernelshap_error}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/kernelshap_insertion_deletion.tex <==
\begin{table}[t]
\centering
\caption{Comparing the quality of Shapley value estimates obtained using ViT Shapley and KernelSHAP via insertion/deletion scores. 
} \label{tab:kernelshap_insertdelete}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{tabular}{lcccccc}

\toprule
 & \multicolumn{2}{c}{Target} & \multicolumn{2}{c}{Non-target} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & Ins. (↑) & Del. (↓) & Ins. (↑) & Del. (↓) \\
\midrule
% Attention last & 0.962 (0.004) & 0.793 (0.013) & - & - \\
% Attention rollout & 0.938 (0.005) & 0.880 (0.010) & - & - \\\midrule
% GradCAM (Attn) & 0.938 (0.006) & 0.948 (0.006) & 0.006 (0.001) & 0.014 (0.001) \\
% GradCAM (LN) & 0.914 (0.006) & 0.937 (0.008) & 0.021 (0.002) & 0.005 (0.000) \\
% IntGrad (Pixel) & 0.967 (0.004) & 0.930 (0.008) & 0.008 (0.001) & 0.004 (0.000) \\
% IntGrad (Embed.) & 0.967 (0.004) & 0.930 (0.008) & 0.008 (0.001) & 0.004 (0.000) \\
% Vanilla (Pixel) & 0.938 (0.005) & 0.860 (0.011) & 0.007 (0.001) & 0.014 (0.001) \\
% Vanilla (Embed.) & 0.950 (0.004) & 0.808 (0.013) & 0.006 (0.001) & 0.020 (0.001) \\
% SmoothGrad (Pixel) & 0.960 (0.005) & 0.779 (0.013) & 0.005 (0.001) & 0.024 (0.001) \\
% SmoothGrad (Embed.) & 0.947 (0.005) & 0.942 (0.006) & 0.006 (0.001) & 0.006 (0.001) \\
% VarGrad (Pixel) & 0.958 (0.005) & 0.796 (0.013) & 0.005 (0.001) & 0.022 (0.001) \\
% VarGrad (Embed.) & 0.949 (0.005) & 0.946 (0.005) & 0.006 (0.001) & 0.006 (0.001) \\
% LRP & 0.967 (0.004) & 0.779 (0.014) & 0.004 (0.001) & 0.022 (0.001) \\\midrule
% Leave-one-out & 0.969 (0.002) & 0.917 (0.010) & 0.013 (0.002) & 0.003 (0.000) \\
% RISE & 0.977 (0.001) & 0.860 (0.014) & 0.023 (0.003) & 0.002 (0.000) \\
ViT Shapley & 0.985 (0.002) & 0.691 (0.014) & 0.093 (0.004) & 0.001 (0.000) \\
KernelSHAP & 0.990 (0.002) & 0.589 (0.053) & 0.158 (0.021) & 0.001 (0.000) \\%\midrule
% Random & 0.951 (0.005) & 0.951 (0.005) & 0.005 (0.001) & 0.005 (0.001) \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\end{table}

==> ViT Shapley (ICLR 2023)/figures/metrics.tex <==
\begin{table}[t]
\centering
% \vspace{-.2cm}
\vskip - 0.4cm
\caption{Evaluating ViT Shapley using standard explanation metrics, with explanations calculated for the target class only. Methods that fail to outperform the random baseline are shown in gray, and the best results are shown in bold (accounting for 95\% confidence intervals).
} \label{tab:metrics}
\begin{center}
{\tablesize
    \begin{tabular}{lcccccc}
    \toprule
     & \multicolumn{3}{c}{ImageNette} & \multicolumn{3}{c}{MURA} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
     & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
    \midrule
    Attention last & 0.962 (0.004) & 0.793 (0.013) & \textbf{0.694 (0.015)} & 0.890 (0.010) & 0.592 (0.013) & 0.635 (0.016) \\
    Attention rollout & \textcolor{gray}{0.938 (0.005)} & 0.880 (0.010) & \textbf{0.704 (0.015)} & \textcolor{gray}{0.845 (0.011)} & 0.692 (0.014) & 0.618 (0.016) \\\midrule
    GradCAM & \textcolor{gray}{0.914 (0.006)} & 0.937 (0.008) & 0.680 (0.015) & 0.899 (0.009) & 0.681 (0.015) & 0.631 (0.016) \\
    IntGrad & 0.967 (0.004) & 0.930 (0.008) & 0.403 (0.024) & 0.897 (0.010) & 0.796 (0.015) & 0.201 (0.022) \\
    Vanilla & \textcolor{gray}{0.950 (0.004)} & 0.808 (0.013) & \textbf{0.703 (0.015)} & 0.890 (0.010) & 0.537 (0.014) & 0.629 (0.016) \\
    SmoothGrad & \textcolor{gray}{0.947 (0.005)} & \textcolor{gray}{0.942 (0.006)} & \textbf{0.703 (0.015)} & 0.870 (0.010) & 0.813 (0.011) & 0.617 (0.016) \\
    VarGrad & \textcolor{gray}{0.949 (0.005)} & \textcolor{gray}{0.946 (0.005)} & \textbf{0.700 (0.015)} & \textcolor{gray}{0.857 (0.011)} & 0.823 (0.011) & 0.615 (0.016) \\
    LRP & 0.967 (0.004) & 0.779 (0.014) & \textbf{0.705 (0.015)} & 0.900 (0.009) & 0.551 (0.013) & 0.646 (0.016) \\\midrule
    Leave-one-out & 0.969 (0.002) & 0.917 (0.010) & 0.140 (0.040) & 0.926 (0.008) & 0.694 (0.017) & 0.308 (0.032) \\
    RISE & 0.977 (0.001) & 0.860 (0.014) & \textbf{0.704 (0.015)} & 0.957 (0.004) & 0.573 (0.018) & 0.618 (0.016) \\
    \textbf{ViT Shapley} & \textbf{0.985 (0.002)} & \textbf{0.691 (0.014)} & \textbf{0.711 (0.015)} & \textbf{0.971 (0.002)} & \textbf{0.307 (0.013)} & \textbf{0.707 (0.013)} \\\midrule
    Random & \textcolor{gray}{0.951 (0.005)} & \textcolor{gray}{0.951 (0.005)} & - & \textcolor{gray}{0.849 (0.010)} & \textcolor{gray}{0.847 (0.010)} & - \\
    \bottomrule
    \end{tabular}
}
\end{center}
\end{table}

==> ViT Shapley (ICLR 2023)/figures/metrics_mura_nontarget.tex <==
\begin{table}[t]
\centering
\caption{
MURA non-target metrics for images that were predicted to be normal. Methods that fail to outperform the random baseline are shown in gray, and the best results are shown in bold (accounting for 95\% confidence intervals).
} \label{tab:metrics_mura_nontarget}
\vskip 0.1in
\begin{center}
% \begin{small}
% \begin{scriptsize}
{\tablesize
    \begin{tabular}{lccc}
    \toprule
     & \multicolumn{3}{c}{MURA} \\
    \cmidrule(lr){2-4} 
     & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
    \midrule
    
    
    Attention last & \textcolor{gray}{0.157 (0.011)} & \textcolor{gray}{0.210 (0.009)} & -0.455 (0.022) \\
    Attention rollout & 0.199 (0.011) & \textcolor{gray}{0.169 (0.010)} & -0.480 (0.023) \\\midrule
    GradCAM & 0.197 (0.012) & \textcolor{gray}{0.152 (0.010)} & -0.449 (0.022) \\
    IntGrad & 0.209 (0.014) & \textcolor{gray}{0.151 (0.010)} & 0.103 (0.023) \\
    Vanilla & \textcolor{gray}{0.174 (0.011)} & \textcolor{gray}{0.197 (0.009)} & -0.477 (0.023) \\
    SmoothGrad & \textcolor{gray}{0.169 (0.011)} & \textcolor{gray}{0.176 (0.011)} & -0.480 (0.023) \\
    VarGrad & \textcolor{gray}{0.166 (0.011)} & \textcolor{gray}{0.175 (0.011)} & -0.478 (0.023) \\
    LRP & \textcolor{gray}{0.169 (0.012)} & \textcolor{gray}{0.200 (0.009)} & -0.461 (0.023) \\\midrule
    Leave-one-out & 0.326 (0.016) & 0.093 (0.007) & 0.272 (0.029) \\
    RISE & 0.406 (0.018) & 0.075 (0.006) & -0.479 (0.023) \\
    \textbf{ViT Shapley} & \textbf{0.580 (0.016)} & \textbf{0.039 (0.003)} & \textbf{0.642 (0.014)} \\\midrule
    Random & \textcolor{gray}{0.169 (0.011)} & \textcolor{gray}{0.170 (0.011)} & - \\    
    \bottomrule
    \end{tabular}
}
% \end{scriptsize}
% \end{small}
\end{center}
\end{table}

==> ViT Shapley (ICLR 2023)/figures/metrics_nontarget.tex <==
% \begin{table}[t]
% \caption{Evaluating ViT Shapley when explaining non-target classes. The metrics are averaged across all non-target classes, and the best-performing methods are shown in bold.
% % for 1,000 ImageNette examples randomly chosen from the test set.
% }
% \vskip 0.1in
% \begin{center}
% \begin{small}
% \begin{tabular}{lccc}
% \toprule
%  & \multicolumn{3}{c}{ImageNette} \\
% \cmidrule(lr){2-4}
%  & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
% \midrule
% Attention last & - & - & - \\
% Attention rollout & - & - & - \\\midrule
% GradCAM & 0.006 (0.001) & 0.014 (0.001) & -0.651 (0.014) \\
% Integrated Gradients & 0.008 (0.001) & 0.004 (0.000) & 0.294 (0.022) \\
% Saliency & 0.006 (0.001) & 0.020 (0.001) & -0.682 (0.015) \\
% SmoothGrad & 0.006 (0.001) & 0.006 (0.001) & -0.683 (0.015) \\
% VarGrad & 0.006 (0.001) & 0.006 (0.001) & -0.680 (0.015) \\
% LRP & 0.004 (0.001) & 0.022 (0.001) & -0.680 (0.015) \\\midrule
% Leave-one-out & 0.013 (0.002) & 0.003 (0.000) & -0.017 (0.028) \\
% RISE & 0.023 (0.003) & 0.002 (0.000) & -0.681 (0.015) \\
% \textbf{ViT Shapley} & \textbf{0.093 (0.004)} & \textbf{0.001 (0.000)} & \textbf{0.672 (0.014)} \\\midrule
% Random & 0.005 (0.001) & 0.005 (0.001) & - \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \end{table}

% \begin{table}[t]
% \caption{Evaluating ViT Shapley when explaining non-target classes. The metrics are averaged across all non-target classes,
% % the best-performing methods are shown in bold, and
% methods that fail to outperform the random baseline
% % on par with random
% are shown in gray, and the best-performing methods are shown in bold.
% % for 1,000 ImageNette examples randomly chosen from the test set.
% } \label{tab:metrics_nontarget}
% \vskip 0.1in
% \begin{center}
% \begin{small}
% \begin{tabular}{lccc}
% \toprule
%  & \multicolumn{3}{c}{ImageNette} \\
% \cmidrule(lr){2-4}
%  & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
% \midrule
% Attention last & - & - & - \\
% Attention rollout & - & - & - \\\midrule
% GradCAM & \textcolor{gray}{0.006 (0.001)} & \textcolor{gray}{0.014 (0.001)} & -0.651 (0.014) \\
% Integrated Gradients & 0.008 (0.001) & 0.004 (0.000) & 0.294 (0.022) \\
% Saliency & \textcolor{gray}{0.006 (0.001)} & \textcolor{gray}{0.020 (0.001)} & -0.682 (0.015) \\
% SmoothGrad & \textcolor{gray}{0.006 (0.001)} & \textcolor{gray}{0.006 (0.001)} & -0.683 (0.015) \\
% VarGrad & \textcolor{gray}{0.006 (0.001)} & \textcolor{gray}{0.006 (0.001)} & -0.680 (0.015) \\
% LRP & \textcolor{gray}{0.004 (0.001)} & \textcolor{gray}{0.022 (0.001)} & -0.680 (0.015) \\\midrule
% Leave-one-out & 0.013 (0.002) & 0.003 (0.000) & -0.017 (0.028) \\
% RISE & 0.023 (0.003) & 0.002 (0.000) & -0.681 (0.015) \\
% \textbf{ViT Shapley} & \textbf{0.093 (0.004)} & \textbf{0.001 (0.000)} & \textbf{0.672 (0.014)} \\\midrule
% Random & \textcolor{gray}{0.005 (0.001)} & \textcolor{gray}{0.005 (0.001)} & - \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \end{table}

% \begin{wraptable}{r}{0.59\textwidth}
% \begin{wraptable}[22]{r}{0.59\textwidth}
    % \vskip -0.18in
\begin{wraptable}[22]{r}{0.59\textwidth}
    \vskip -0.15in
    \caption{Evaluating ViT Shapley for explaining non-target classes.
    % The metrics are averaged across all non-target classes,
    % the best-performing methods are shown in bold, and
    Methods that fail to outperform the random baseline
    % on par with random
    are shown in gray, and the best results are
    % bolded.
    % -performing methods are
    shown in bold (accounting for 95\% confidence intervals).
    % for 1,000 ImageNette examples randomly chosen from the test set.
    } \label{tab:metrics_nontarget}
    % \begin{table}[t]
    \vskip 0.1in
    \begin{center}
    % \begin{small}
    {\tablesize
        \begin{tabular}{lccc}
        \toprule
         & \multicolumn{3}{c}{ImageNette} \\
        \cmidrule(lr){2-4}
         & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
        \midrule
        Attention last & - & - & - \\
        Attention rollout & - & - & - \\\midrule
        GradCAM & 0.021 (0.002) & \textcolor{gray}{0.005 (0.000)} & -0.672 (0.015) \\
        IntGrad & 0.008 (0.001) & 0.004 (0.000) & 0.294 (0.022) \\
        Vanilla & \textcolor{gray}{0.006 (0.001)} & \textcolor{gray}{0.020 (0.001)} & -0.682 (0.015) \\
        SmoothGrad & \textcolor{gray}{0.006 (0.001)} & \textcolor{gray}{0.006 (0.001)} & -0.683 (0.015) \\
        VarGrad & \textcolor{gray}{0.006 (0.001)} & \textcolor{gray}{0.006 (0.001)} & -0.680 (0.015) \\
        LRP & \textcolor{gray}{0.004 (0.001)} & \textcolor{gray}{0.022 (0.001)} & -0.680 (0.015) \\\midrule
        Leave-one-out & 0.013 (0.002) & 0.003 (0.000) & -0.017 (0.028) \\
        RISE & 0.023 (0.003) & 0.002 (0.000) & -0.681 (0.015) \\
        \textbf{ViT Shapley} & \textbf{0.093 (0.004)} & \textbf{0.001 (0.000)} & \textbf{0.672 (0.014)} \\\midrule
        Random & \textcolor{gray}{0.005 (0.001)} & \textcolor{gray}{0.005 (0.001)} & - \\
        \bottomrule
        \end{tabular}
    }
    % \end{small}
    \end{center}
    % \end{table}
\end{wraptable}

==> ViT Shapley (ICLR 2023)/figures/metrics_supplement_direct_masking.tex <==
\begin{table}[t]
\centering
\caption{Performance metrics for target classes explanations
for a ViT classifier trained with random masking. Methods that fail to outperform the random baseline are shown in gray, and the best results are shown in bold (accounting for 95\% confidence intervals).
} \label{tab:metrics_supplement_direct_masking}
\vskip 0.1in
\begin{center}
{\tablesize
    \begin{tabular}{lccc}
    \toprule
     & \multicolumn{3}{c}{ImageNette} \\
    \cmidrule(lr){2-4}
     & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
    \midrule
%0.588
    Attention last & \textcolor{gray}{0.963 (0.003)} & 0.839 (0.011) & \textbf{0.593 (0.017)} \\
    Attention rollout & \textcolor{gray}{0.945 (0.004)} & 0.903 (0.008) & \textbf{0.597 (0.017)} \\\midrule
    GradCAM (LN) & \textcolor{gray}{0.955 (0.003)} & 0.898 (0.011) & \textbf{0.585 (0.016)} \\
    GradCAM (Attn) & \textcolor{gray}{0.945 (0.005)} & 0.942 (0.006) & 0.564 (0.016) \\
    IntGrad (Pixel) & 0.977 (0.002) & 0.933 (0.008) & 0.474 (0.017) \\
    IntGrad (Embed.) & 0.977 (0.002) & 0.933 (0.008) & 0.474 (0.017) \\
    Vanilla (Pixel) & \textcolor{gray}{0.934 (0.005)} & 0.901 (0.009) & \textbf{0.593 (0.017)} \\
    Vanilla (Embed.) & \textcolor{gray}{0.948 (0.004)} & 0.864 (0.011) & \textbf{0.595 (0.017)} \\
    SmoothGrad (Pixel) & 0.966 (0.004) & 0.809 (0.012) & \textbf{0.599 (0.017)} \\
    SmoothGrad (Embed.) & \textcolor{gray}{0.954 (0.004)} & \textcolor{gray}{0.950 (0.005)} & \textbf{0.597 (0.017)} \\
    VarGrad (Pixel) & 0.964 (0.004) & 0.826 (0.011) & \textbf{0.573 (0.016)} \\
    VarGrad (Embed.) & \textcolor{gray}{0.953 (0.005)} & \textcolor{gray}{0.954 (0.004)} & \textbf{0.594 (0.017)} \\
    LRP & 0.972 (0.002) & 0.806 (0.013) & \textbf{0.603 (0.017)} \\\midrule
    Leave-one-out & 0.977 (0.001) & 0.881 (0.014) & 0.134 (0.034) \\
    RISE & 0.982 (0.001) & 0.793 (0.017) & \textbf{0.599 (0.017)} \\
    \textbf{ViT Shapley} & \textbf{0.988 (0.001)} & \textbf{0.736 (0.013)} & \textbf{0.605 (0.017)} \\\midrule
    Random & \textcolor{gray}{0.957 (0.004)} & \textcolor{gray}{0.957 (0.004)} & - \\
    
    \bottomrule
    \end{tabular}
}
\end{center}
\end{table}

==> ViT Shapley (ICLR 2023)/figures/metrics_supplement_pet.tex <==
\begin{table}[t]
\centering
\caption{Performance metrics
% for explanations
% the target class only
% with additional baselines on
for ViT-Base on Pets. Methods that fail to outperform the random baseline are shown in gray, and the best results are shown in bold (accounting for 95\% confidence intervals).
} \label{tab:metrics_supplement_pet}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{scriptsize}
{\tablesize
    \begin{tabular}{lcccccc}
    \toprule
     & \multicolumn{3}{c}{Target} & \multicolumn{3}{c}{Non-Target} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
     & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
    \midrule
    Attention last & 0.876 (0.011) & 0.494 (0.016) & 0.545 (0.017) & - & - & - \\
    Attention rollout & \textcolor{gray}{0.837 (0.012)} & 0.672 (0.017) & \textbf{0.559 (0.017)} & - & - & - \\\midrule
    GradCAM (Attn) & \textcolor{gray}{0.837 (0.013)} & 0.737 (0.018) & 0.527 (0.016) & \textcolor{gray}{0.005 (0.000)} & \textcolor{gray}{0.008 (0.000)} & -0.499 (0.013) \\
    GradCAM (LN) & \textcolor{gray}{0.837 (0.011)} & 0.717 (0.019) & 0.553 (0.017) & 0.012 (0.001) & 0.004 (0.000) & -0.511 (0.014) \\
    IntGrad (Pixel) & 0.899 (0.010) & 0.802 (0.016) & 0.437 (0.017) & 0.006 (0.001) & 0.003 (0.000) & 0.126 (0.008) \\
    IntGrad (Embed.) & 0.899 (0.010) & 0.802 (0.016) & 0.437 (0.017) & 0.006 (0.001) & 0.003 (0.000) & 0.126 (0.008) \\
    Vanilla (Pixel) & \textcolor{gray}{0.862 (0.011)} & 0.596 (0.018) & \textbf{0.559 (0.017)} & \textcolor{gray}{0.004 (0.000)} & \textcolor{gray}{0.011 (0.000)} & -0.526 (0.014) \\
    Vanilla (Embed.) & 0.876 (0.011) & 0.519 (0.017) & \textbf{0.561 (0.017)} & \textcolor{gray}{0.004 (0.000)} & \textcolor{gray}{0.013 (0.000)} & -0.529 (0.014) \\
    SmoothGrad (Pixel) & 0.889 (0.011) & 0.488 (0.016) & \textbf{0.564 (0.017)} & \textcolor{gray}{0.003 (0.000)} & \textcolor{gray}{0.014 (0.000)} & -0.532 (0.014) \\
    SmoothGrad (Embed.) & \textcolor{gray}{0.840 (0.013)} & \textcolor{gray}{0.834 (0.013)} & \textbf{0.558 (0.017)} & \textcolor{gray}{0.004 (0.000)} & \textcolor{gray}{0.005 (0.000)} & -0.526 (0.014) \\
    VarGrad (Pixel) & 0.891 (0.011) & 0.513 (0.016) & \textbf{0.557 (0.017)} & \textcolor{gray}{0.003 (0.000)} & \textcolor{gray}{0.013 (0.000)} & -0.522 (0.014) \\
    VarGrad (Embed.) & \textcolor{gray}{0.847 (0.012)} & \textcolor{gray}{0.835 (0.013)} & 0.555 (0.017) & \textcolor{gray}{0.004 (0.000)} & \textcolor{gray}{0.005 (0.000)} & -0.523 (0.014) \\
    LRP & 0.890 (0.011) & 0.466 (0.016) & \textbf{0.567 (0.017)} & \textcolor{gray}{0.004 (0.000)} & \textcolor{gray}{0.013 (0.000)} & -0.529 (0.014) \\\midrule
    Leave-one-out & \textbf{0.936 (0.006)} & 0.653 (0.022) & 0.215 (0.036) & 0.018 (0.001) & 0.001 (0.000) & 0.138 (0.023) \\
    RISE & \textbf{0.946 (0.005)} & 0.505 (0.022) & \textbf{0.559 (0.017)} & 0.032 (0.002) & 0.001 (0.000) & -0.523 (0.014) \\
    \textbf{ViT Shapley} & \textbf{0.945 (0.006)} & \textbf{0.388 (0.017)} & \textbf{0.590 (0.016)} & \textbf{0.052 (0.002)} & \textbf{0.001 (0.000)} & \textbf{0.529 (0.012)} \\\midrule
    Random & \textcolor{gray}{0.848 (0.012)} & \textcolor{gray}{0.845 (0.012)} & - & \textcolor{gray}{0.004 (0.000)} & \textcolor{gray}{0.004 (0.000)} & - \\
    \bottomrule
    \end{tabular}
}
% \end{scriptsize}
\end{small}
\end{center}
\end{table}

==> ViT Shapley (ICLR 2023)/figures/metrics_supplement_vitlarge.tex <==
\begin{table}[t]
\centering
\caption{Performance metrics
% for explanations
% the target class only
% with additional baselines on
for ViT-Large on ImageNette. Methods that fail to outperform the random baseline are shown in gray, and the best results are shown in bold (accounting for 95\% confidence intervals).
} \label{tab:metrics_supplement_vitlarge}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{scriptsize}
{\tablesize
    \begin{tabular}{lcccccc}
    \toprule
     & \multicolumn{3}{c}{Target} & \multicolumn{3}{c}{Non-Target} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
     & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
    \midrule
    Attention last & \textcolor{gray}{0.915 (0.005)} & 0.896 (0.008) & 0.401 (0.022) & - & - & - \\
    Attention rollout & \textcolor{gray}{0.929 (0.005)} & 0.928 (0.007) & \textbf{0.423 (0.023)} & - & - & - \\\midrule
    GradCAM (LN) & \textcolor{gray}{0.955 (0.004)} & 0.924 (0.009) & \textbf{0.424 (0.023)} & 0.012 (0.001) & \textcolor{gray}{0.005 (0.000)} & -0.372 (0.020) \\
    GradCAM (Attn) & \textcolor{gray}{0.935 (0.005)} & 0.930 (0.007) & 0.395 (0.022) & 0.007 (0.001) & \textcolor{gray}{0.006 (0.001)} & -0.351 (0.018) \\
    IntGrad (Pixel) & 0.965 (0.003) & \textcolor{gray}{0.947 (0.006)} & 0.195 (0.020) & \textcolor{gray}{0.006 (0.001)} & 0.004 (0.000) & 0.114 (0.013) \\
    IntGrad (Embed.) & 0.965 (0.003) & \textcolor{gray}{0.948 (0.006)} & 0.198 (0.020) & \textcolor{gray}{0.006 (0.001)} & 0.004 (0.000) & 0.117 (0.013) \\
    Vanilla (Pixel) & \textcolor{gray}{0.898 (0.007)} & 0.921 (0.007) & \textbf{0.411 (0.022)} & 0.012 (0.001) & \textcolor{gray}{0.008 (0.001)} & -0.370 (0.020) \\
    Vanilla (Embed.) & \textcolor{gray}{0.911 (0.006)} & 0.905 (0.009) & \textbf{0.415 (0.023)} & 0.010 (0.001) & \textcolor{gray}{0.010 (0.001)} & -0.373 (0.020) \\
    SmoothGrad (Pixel) & \textcolor{gray}{0.949 (0.004)} & 0.861 (0.011) & \textbf{0.424 (0.023)} & 0.006 (0.001) & \textcolor{gray}{0.014 (0.001)} & -0.382 (0.020) \\
    SmoothGrad (Embed.) & \textcolor{gray}{0.956 (0.004)} & 0.857 (0.011) & \textbf{0.423 (0.023)} & \textcolor{gray}{0.005 (0.000)} & \textcolor{gray}{0.015 (0.001)} & -0.380 (0.020) \\
    VarGrad (Pixel) & \textcolor{gray}{0.942 (0.005)} & 0.878 (0.010) & 0.387 (0.021) & 0.007 (0.001) & \textcolor{gray}{0.013 (0.001)} & -0.350 (0.018) \\
    VarGrad (Embed.) & \textcolor{gray}{0.944 (0.005)} & 0.875 (0.010) & 0.383 (0.020) & 0.007 (0.001) & \textcolor{gray}{0.013 (0.001)} & -0.343 (0.017) \\
    LRP & \textcolor{gray}{0.946 (0.004)} & 0.869 (0.010) & \textbf{0.424 (0.023)} & 0.006 (0.001) & \textcolor{gray}{0.013 (0.001)} & -0.381 (0.020) \\\midrule
    Leave-one-out & 0.970 (0.003) & 0.938 (0.007) & 0.123 (0.031) & 0.009 (0.001) & 0.003 (0.000) & 0.118 (0.020) \\
    RISE & 0.978 (0.002) & 0.882 (0.013) & \textbf{0.425 (0.023)} & 0.019 (0.003) & 0.002 (0.000) & -0.381 (0.020) \\
    \textbf{ViT Shapley} & \textbf{0.986 (0.002)} & \textbf{0.742 (0.013)} & \textbf{0.439 (0.023)} & \textbf{0.077 (0.003)} & \textbf{0.001 (0.000)} & \textbf{0.391 (0.019)} \\\midrule
    Random & \textcolor{gray}{0.957 (0.004)} & \textcolor{gray}{0.956 (0.004)} & - & \textcolor{gray}{0.005 (0.000)} & \textcolor{gray}{0.005 (0.000)} & - \\
    \bottomrule
    \end{tabular}
}
% \end{scriptsize}
\end{small}
\end{center}
\end{table}

==> ViT Shapley (ICLR 2023)/figures/metrics_supplement_vitsmall.tex <==
\begin{table}[t]
\centering
\caption{Performance metrics
% for explanations
% the target class only
% with additional baselines on
for ViT-Small on ImageNette. Methods that fail to outperform the random baseline are shown in gray, and the best results are shown in bold (accounting for 95\% confidence intervals).
} \label{tab:metrics_supplement_vitsmall}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{scriptsize}
{\tablesize
    \begin{tabular}{lcccccc}
    \toprule
     & \multicolumn{3}{c}{Target} & \multicolumn{3}{c}{Non-Target} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
     & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
    \midrule
    Attention last & 0.949 (0.006) & 0.706 (0.014) & \textbf{0.781 (0.011)} & - & - & - \\
    Attention rollout & \textcolor{gray}{0.914 (0.007)} & 0.814 (0.013) & \textbf{0.787 (0.011)} & - & - & - \\\midrule
    GradCAM (LN) & \textcolor{gray}{0.908 (0.006)} & 0.898 (0.011) & 0.770 (0.010) & 0.027 (0.002) & 0.006 (0.000) & -0.740 (0.009) \\
    GradCAM (Attn.) & \textcolor{gray}{0.904 (0.009)} & 0.911 (0.009) & 0.724 (0.010) & \textcolor{gray}{0.008 (0.001)} & \textcolor{gray}{0.016 (0.001)} & -0.717 (0.009) \\
    IntGrad (Pixel) & 0.951 (0.006) & 0.908 (0.010) & 0.541 (0.022) & 0.011 (0.001) & 0.005 (0.001) & 0.384 (0.018) \\
    IntGrad (Embed.) & 0.951 (0.006) & 0.908 (0.010) & 0.541 (0.022) & 0.011 (0.001) & 0.005 (0.001) & 0.384 (0.018) \\
    Vanilla (Pixel) & \textcolor{gray}{0.905 (0.007)} & 0.830 (0.012) & \textbf{0.784 (0.010)} & 0.011 (0.001) & \textcolor{gray}{0.018 (0.001)} & -0.754 (0.009) \\
    Vanilla (Embed.) & \textcolor{gray}{0.921 (0.007)} & 0.793 (0.013) & \textbf{0.786 (0.011)} & 0.009 (0.001) & \textcolor{gray}{0.022 (0.001)} & -0.756 (0.009) \\
    SmoothGrad (Pixel) & \textcolor{gray}{0.943 (0.006)} & 0.744 (0.014) & \textbf{0.786 (0.011)} & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.027 (0.001)} & -0.756 (0.009) \\
    SmoothGrad (Embed.) & 0.946 (0.006) & 0.753 (0.014) & \textbf{0.787 (0.011)} & \textcolor{gray}{0.006 (0.001)} & \textcolor{gray}{0.026 (0.001)} & -0.757 (0.009) \\
    VarGrad (Pixel) & 0.946 (0.006) & 0.766 (0.013) & 0.742 (0.010) & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.025 (0.001)} & -0.709 (0.009) \\
    VarGrad (Embed.) & 0.947 (0.006) & 0.774 (0.013) & 0.758 (0.010) & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.024 (0.001)} & -0.723 (0.009) \\
    LRP & 0.957 (0.005) & 0.695 (0.015) & \textbf{0.793 (0.010)} & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.027 (0.001)} & -0.753 (0.009) \\\midrule
    Leave-one-out & 0.967 (0.002) & 0.855 (0.015) & 0.044 (0.042) & 0.024 (0.002) & 0.003 (0.000) & 0.079 (0.030) \\
    RISE & 0.976 (0.002) & 0.752 (0.018) & \textbf{0.787 (0.010)} & 0.049 (0.004) & 0.002 (0.000) & -0.755 (0.009) \\
    \textbf{ViT Shapley} & \textbf{0.982 (0.002)} & \textbf{0.591 (0.015)} & \textbf{0.801 (0.010)} & \textbf{0.130 (0.005)} & \textbf{0.001 (0.000)} & \textbf{0.747 (0.009)} \\\midrule
    Random & \textcolor{gray}{0.933 (0.006)} & \textcolor{gray}{0.934 (0.006)} & - & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.007 (0.001)} & - \\
    \bottomrule
    \end{tabular}
}
% \end{scriptsize}
\end{small}
\end{center}
\end{table}

==> ViT Shapley (ICLR 2023)/figures/metrics_supplement_vitsmall_nontarget.tex <==
\begin{table}[t]
\centering
\caption{Performance metrics for non-target classes explanations
% the target class only
% with additional baselines on
with the ViT-Small architecture. Methods that fail to outperform the random baseline are shown in gray, and the best results are shown in bold (accounting for 95\% confidence intervals).
} \label{tab:metrics_supplement_vitsmall_nontarget}
\vskip 0.1in
\begin{center}
% \begin{small}
% \begin{scriptsize}
{\tablesize
    \begin{tabular}{lccc}
    \toprule
     & \multicolumn{3}{c}{ImageNette} \\
    \cmidrule(lr){2-4}
     & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
    \midrule
    Attention last & - & - & - \\
    Attention rollout & - & - & - \\\midrule
    GradCAM (LN) & 0.027 (0.002) & 0.006 (0.000) & -0.740 (0.009) \\
    GradCAM (Attn.) & \textcolor{gray}{0.008 (0.001)} & \textcolor{gray}{0.016 (0.001)} & -0.717 (0.009) \\
    IntGrad (Pixel) & 0.011 (0.001) & 0.005 (0.001) & 0.384 (0.018) \\
    IntGrad (Embed.) & 0.011 (0.001) & 0.005 (0.001) & 0.384 (0.018) \\
    Vanilla (Pixel) & 0.011 (0.001) & \textcolor{gray}{0.018 (0.001)} & -0.754 (0.009) \\
    Vanilla (Embed.) & 0.009 (0.001) & \textcolor{gray}{0.022 (0.001)} & -0.756 (0.009) \\
    SmoothGrad (Pixel) & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.027 (0.001)} & -0.756 (0.009) \\
    SmoothGrad (Embed.) & \textcolor{gray}{0.006 (0.001)} & \textcolor{gray}{0.026 (0.001)} & -0.757 (0.009) \\
    VarGrad (Pixel) & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.025 (0.001)} & -0.709 (0.009) \\
    VarGrad (Embed.) & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.024 (0.001)} & -0.723 (0.009) \\
    LRP & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.027 (0.001)} & -0.753 (0.009) \\\midrule
    Leave-one-out & 0.024 (0.002) & 0.003 (0.000) & 0.079 (0.030) \\
    RISE & 0.049 (0.004) & 0.002 (0.000) & -0.755 (0.009) \\
    \textbf{ViT Shapley} & \textbf{0.130 (0.005)} & \textbf{0.001 (0.000)} & \textbf{0.747 (0.009)} \\\midrule
    Random & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.007 (0.001)} & - \\
    \bottomrule
    \end{tabular}
}
% \end{scriptsize}
% \end{small}
\end{center}
\end{table}

==> ViT Shapley (ICLR 2023)/figures/metrics_supplement_vitsmall_target.tex <==
\begin{table}[t]
\centering
\caption{Performance metrics for target classes explanations
% the target class only
% with additional baselines on
with the ViT-Small architecture. Methods that fail to outperform the random baseline are shown in gray, and the best results are shown in bold (accounting for 95\% confidence intervals).
} \label{tab:metrics_supplement_vitsmall_target}
\vskip 0.1in
\begin{center}
% \begin{small}
% \begin{scriptsize}
{\tablesize
    \begin{tabular}{lccc}
    \toprule
     & \multicolumn{3}{c}{ImageNette} \\
    \cmidrule(lr){2-4}
     & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
    \midrule
    Attention last & 0.949 (0.006) & 0.706 (0.014) & \textbf{0.781 (0.011)} \\
    Attention rollout & \textcolor{gray}{0.914 (0.007)} & 0.814 (0.013) & \textbf{0.787 (0.011)} \\\midrule
    GradCAM (LN) & \textcolor{gray}{0.908 (0.006)} & 0.898 (0.011) & 0.770 (0.010) \\
    GradCAM (Attn.) & \textcolor{gray}{0.904 (0.009)} & 0.911 (0.009) & 0.724 (0.010) \\
    IntGrad (Pixel) & 0.951 (0.006) & 0.908 (0.010) & 0.541 (0.022) \\
    IntGrad (Embed.) & 0.951 (0.006) & 0.908 (0.010) & 0.541 (0.022) \\
    Vanilla (Pixel) & \textcolor{gray}{0.905 (0.007)} & 0.830 (0.012) & \textbf{0.784 (0.010)} \\
    Vanilla (Embed.) & \textcolor{gray}{0.921 (0.007)} & 0.793 (0.013) & \textbf{0.786 (0.011)} \\
    SmoothGrad (Pixel) & \textcolor{gray}{0.943 (0.006)} & 0.744 (0.014) & \textbf{0.786 (0.011)} \\
    SmoothGrad (Embed.) & 0.946 (0.006) & 0.753 (0.014) & \textbf{0.787 (0.011)} \\
    VarGrad (Pixel) & 0.946 (0.006) & 0.766 (0.013) & 0.742 (0.010) \\
    VarGrad (Embed.) & 0.947 (0.006) & 0.774 (0.013) & 0.758 (0.010) \\
    LRP & 0.957 (0.005) & 0.695 (0.015) & \textbf{0.793 (0.010)} \\\midrule
    Leave-one-out & 0.967 (0.002) & 0.855 (0.015) & 0.044 (0.042) \\
    RISE & 0.976 (0.002) & 0.752 (0.018) & \textbf{0.787 (0.010)} \\
    \textbf{ViT Shapley} & \textbf{0.982 (0.002)} & \textbf{0.591 (0.015)} & \textbf{0.801 (0.010)} \\\midrule
    Random & \textcolor{gray}{0.933 (0.006)} & \textcolor{gray}{0.934 (0.006)} & - \\
    \bottomrule
    \end{tabular}
}
% \end{scriptsize}
% \end{small}
\end{center}
\end{table}

==> ViT Shapley (ICLR 2023)/figures/metrics_supplement_vittiny.tex <==
\begin{table}[t]
\centering
\caption{Performance metrics
% for explanations
% the target class only
% with additional baselines on
for ViT-Tiny on ImageNette. Methods that fail to outperform the random baseline are shown in gray, and the best results are shown in bold (accounting for 95\% confidence intervals).
} \label{tab:metrics_supplement_vittiny}
\vskip 0.1in
\begin{center}
% \begin{small}
% \begin{scriptsize}
{\tablesize
    \begin{tabular}{lcccccc}
    \toprule
     & \multicolumn{3}{c}{Target} & \multicolumn{3}{c}{Non-Target} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
     & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
    \midrule
    % \toprule
    % & \multicolumn{3}{c}{Target} \multicolumn{3}{c}{Non-target} \\
    % \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    %  & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
    % \midrule
    Attention last & \textcolor{gray}{0.917 (0.008)} & 0.702 (0.015) & 0.649 (0.014) & - & - & - \\
    Attention rollout & \textcolor{gray}{0.901 (0.009)} & 0.698 (0.015) & 0.658 (0.015) & - & - & - \\\midrule
    GradCAM (LN) & \textcolor{gray}{0.918 (0.007)} & 0.809 (0.014) & 0.659 (0.014) & 0.034 (0.002) & 0.006 (0.000) & -0.616 (0.013) \\
    GradCAM (Attn) & \textcolor{gray}{0.898 (0.009)} & 0.814 (0.013) & 0.636 (0.014) & \textcolor{gray}{0.011 (0.001)} & \textcolor{gray}{0.020 (0.001)} & -0.607 (0.012) \\
    IntGrad (Pixel) & 0.928 (0.006) & 0.852 (0.013) & 0.293 (0.025) & 0.018 (0.002) & 0.008 (0.001) & 0.094 (0.014) \\
    IntGrad (Embed.) & 0.928 (0.006) & 0.852 (0.013) & 0.293 (0.025) & 0.018 (0.002) & 0.008 (0.001) & 0.094 (0.014) \\
    Vanilla (Pixel) & \textcolor{gray}{0.884 (0.009)} & 0.801 (0.013) & 0.656 (0.015) & 0.015 (0.001) & \textcolor{gray}{0.020 (0.001)} & -0.629 (0.013) \\
    Vanilla (Embed.) & \textcolor{gray}{0.902 (0.008)} & 0.752 (0.015) & 0.659 (0.015) & 0.012 (0.001) & \textcolor{gray}{0.025 (0.001)} & -0.632 (0.013) \\
    SmoothGrad (Pixel) & \textcolor{gray}{0.908 (0.009)} & 0.733 (0.015) & 0.659 (0.015) & \textcolor{gray}{0.011 (0.001)} & \textcolor{gray}{0.029 (0.002)} & -0.632 (0.013) \\
    SmoothGrad (Embed.) & \textcolor{gray}{0.917 (0.008)} & 0.756 (0.014) & 0.659 (0.015) & \textcolor{gray}{0.010 (0.001)} & \textcolor{gray}{0.025 (0.002)} & -0.632 (0.013) \\
    VarGrad (Pixel) & \textcolor{gray}{0.914 (0.008)} & 0.754 (0.014) & 0.648 (0.014) & \textcolor{gray}{0.011 (0.001)} & \textcolor{gray}{0.027 (0.002)} & -0.620 (0.012) \\
    VarGrad (Embed.) & \textcolor{gray}{0.921 (0.008)} & 0.777 (0.014) & 0.648 (0.014) & \textcolor{gray}{0.010 (0.001)} & \textcolor{gray}{0.023 (0.001)} & -0.618 (0.012) \\
    LRP & 0.938 (0.007) & 0.648 (0.016) & \textbf{0.673 (0.014)} & 0.014 (0.001) & \textcolor{gray}{0.024 (0.001)} & -0.623 (0.013) \\\midrule
    Leave-one-out & 0.956 (0.004) & 0.737 (0.019) & 0.221 (0.039) & 0.052 (0.004) & 0.003 (0.000) & 0.145 (0.025) \\
    RISE & 0.970 (0.003) & 0.602 (0.019) & 0.658 (0.015) & 0.092 (0.005) & 0.002 (0.000) & -0.628 (0.013) \\
    \textbf{ViT Shapley} & \textbf{0.981 (0.002)} & \textbf{0.457 (0.015)} & \textbf{0.694 (0.014)} & \textbf{0.198 (0.006)} & \textbf{0.001 (0.000)} & \textbf{0.641 (0.011)} \\\midrule
    Random & \textcolor{gray}{0.908 (0.008)} & \textcolor{gray}{0.907 (0.008)} & - & \textcolor{gray}{0.010 (0.001)} & \textcolor{gray}{0.010 (0.001)} & - \\
    \bottomrule
    \end{tabular}
}
% \end{scriptsize}
% \end{small}
\end{center}
\end{table}

==> ViT Shapley (ICLR 2023)/figures/qualitative.tex <==
\begin{figure}[t]
    % \figurespacing
    \vskip -0.6cm
    \centering
    \includegraphics[width=0.95\linewidth]{images/qualitative_three_rows.pdf}
    \vskip -0.2cm
    \caption{
    Explanations where our approach identifies relevant information for target and non-target classes.
    \textbf{Left:} original images from the ImageNette and MURA datasets.
    \textbf{Middle left:} explanations generated by ViT Shapley
    for specific classes.
    \textbf{Right:} probability of the class being explained after the insertion or deletion of important patches (higher is better for insertion, lower for deletion).
    }
    \label{fig:qualitative}
    \vspace{-.2cm}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/qualitative_baselines_imagenette_1.tex <==
\begin{figure}[t]
    \vspace{-.2cm}
    \centering
    \includegraphics[width=1.0\linewidth]{images/qualitative_baselines_ImageNette_0.pdf}
    \caption{
    ViT Shapley vs. baselines comparison (ImageNette).
    }
    \label{fig:qualitative_baselines_imagenette_1}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/qualitative_baselines_imagenette_2.tex <==
\begin{figure}[t]
    \vspace{-.2cm}
    \centering
    \includegraphics[width=1.0\linewidth]{images/qualitative_baselines_ImageNette_1.pdf}
    \caption{
    ViT Shapley vs. baselines comparison (ImageNette).
    }
    \label{fig:qualitative_baselines_imagenette_2}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/qualitative_baselines_imagenette_3.tex <==
\begin{figure}[t]
    \vspace{-.2cm}
    \centering
    \includegraphics[width=1.0\linewidth]{images/qualitative_baselines_ImageNette_3.pdf}
    \caption{
    ViT Shapley vs. baselines comparison (ImageNette).
    }
    \label{fig:qualitative_baselines_imagenette_3}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/qualitative_baselines_mura_1.tex <==
\begin{figure}[t]
    \vspace{-.2cm}
    \centering
    \includegraphics[width=1.0\linewidth]{images/qualitative_baselines_MURA_1.pdf}
    \caption{
    ViT Shapley vs. baselines comparison (MURA).
    }
    \label{fig:qualitative_baselines_MURA_1}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/qualitative_baselines_mura_2.tex <==
\begin{figure}[t]
    \vspace{-.2cm}
    \centering
    \includegraphics[width=1.0\linewidth]{images/qualitative_baselines_MURA_2.pdf}
    \caption{
    ViT Shapley vs. baselines comparison (MURA).
    }
    \label{fig:qualitative_baselines_MURA_2}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/qualitative_baselines_mura_3.tex <==
\begin{figure}[t]
    \vspace{-.2cm}
    \centering
    \includegraphics[width=1.0\linewidth]{images/qualitative_baselines_MURA_4.pdf}
    \caption{
    ViT Shapley vs. baselines comparison (MURA).
    }
    \label{fig:qualitative_baselines_MURA_3}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/qualitative_baselines_nontarget.tex <==
\begin{figure}[t]
     \vspace{-.2cm}
    \centering
    \includegraphics[width=0.3\linewidth]{images/qualitative_baselines_nontarget_1.pdf}
    \includegraphics[width=0.3\linewidth]{images/qualitative_baselines_nontarget_2.pdf}
    \includegraphics[width=0.3\linewidth]{images/qualitative_baselines_nontarget_3.pdf}
    \caption{
    ViT Shapley vs. baselines for non-target classes (ImageNette).
    \textbf{Left:} ViT Shapley shows that the grass in the background provides evidence for the golf ball class.
    \textbf{Middle:} ViT Shapley shows that the sky and its reflection on the water provide evidence for the parachute class.
    \textbf{Right:} ViT Shapley shows that the metallic gas pump handle provides evidence for the French horn class.
    }
    \label{fig:qualitative_baselines_nontarget}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/qualitative_baselines_pet_1.tex <==
\begin{figure}[t]
    \vspace{-.2cm}
    \centering
    \includegraphics[width=1.0\linewidth]{images/qualitative_baselines_Pet_1.pdf}
    \caption{
    ViT Shapley vs. baselines comparison (Pets).
    }
    \label{fig:qualitative_baselines_pet_1}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/qualitative_baselines_pet_2.tex <==
\begin{figure}[t]
    \vspace{-.2cm}
    \centering
    \includegraphics[width=1.0\linewidth]{images/qualitative_baselines_Pet_2.pdf}
    \caption{
    ViT Shapley vs. baselines comparison (Pets).
    }
    \label{fig:qualitative_baselines_pet_2}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/qualitative_baselines_pet_3.tex <==
\begin{figure}[t]
    \vspace{-.2cm}
    \centering
    \includegraphics[width=1.0\linewidth]{images/qualitative_baselines_Pet_3.pdf}
    \caption{
    ViT Shapley vs. baselines comparison (Pets).
    }
    \label{fig:qualitative_baselines_pet_3}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/qualitative_baselines_pet_4.tex <==
\begin{figure}[t]
    \vspace{-.2cm}
    \centering
    \includegraphics[width=1.0\linewidth]{images/qualitative_baselines_Pet_4.pdf}
    \caption{
    ViT Shapley vs. baselines comparison (Pets).
    }
    \label{fig:qualitative_baselines_pet_4}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/qualitative_vit_shapley.tex <==
\begin{figure}[t]
    % \vspace{-.2cm}
    \centering
    \includegraphics[width=0.5\linewidth]{example-image-golden}
    \caption{
    ViT Shapley examples.
    }
    \label{fig:qualitative_vit_shapley}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/removal.tex <==
\begin{figure}[t]
    %\vspace{-.2cm}
    % \vspace{.7cm}
    \figurespacing
    \centering
    %\includegraphics[width=0.9\linewidth]{images/removal.pdf}
    \includegraphics[width=0.9\linewidth]{images/removal_kl.pdf}
    \caption{
    % Measuring
    % a ViT's
    ViT predictions given
    % robustness to
    partial information.
    % held-out patches
    % under different removal schemes.
    % Using the Imagenette and MURA datasets,
    We delete patches at random using several removal mechanisms, and then measure the quality of the resulting predictions via the
    % We make predictions while removing
    % % remove
    % % different numbers of
    % patches at random, and then measure the quality of
    % the resulting predictions.
    % agreement with predictions given the full images.
    % set of image patches.
    %\textbf{Top:}~
    KL divergence relative to
    % with respect to
    the original, full-image
    % full-model
    predictions (lower is better).
    % Similar results for top-1 accuracy are shown in \Cref{app:results}.
    % is shown.
    %\textbf{Bottom:}~accuracy with respect to the true labels.
    % classification agreement with the original predictions.
    }
    \label{fig:removal}
    % \vspace{-.4cm}
    \vspace{-.2cm}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/removal_accuracy.tex <==
\begin{figure}[t]
    \figurespacing
    \centering
    \vskip -0.2in
    \includegraphics[width=1.0\linewidth]{images/removal.pdf}
    \caption{
    ViT predictions given
    % robustness to
    partial information.
    % held-out patches
    % under different removal schemes.
    % Using the Imagenette and MURA datasets,
    We delete patches at random using several removal mechanisms, and we then measure the quality of the resulting predictions via two metrics: the
    % We make predictions while removing
    % % remove
    % % different numbers of
    % patches at random, and then measure the quality of
    % the resulting predictions.
    % agreement with predictions given the full images.
    % set of image patches.
    %\textbf{Top:}~
    KL divergence relative to
    % with respect to
    the original, full-image
    % full-model
    predictions (top), and the top-1 accuracy relative to the true labels (bottom).
    % Similar results for top-1 accuracy are shown in \Cref{app:results}.
    % is shown.
    %\textbf{Bottom:}~accuracy with respect to the true labels.
    % classification agreement with the original predictions.
    }
    \label{fig:removal_accuracy}
    % \vspace{-.4cm}
    % \vspace{-.2cm}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/roar_all.tex <==
\begin{figure}[t]
    % \vspace{-.2cm}
    \figurespacing
    \centering
    \includegraphics[width=\linewidth]{images/roar_all.pdf}
    % \vskip -0.2cm
    \caption{ImageNette accuracy when removing features in order of
    % according to
    their importance, run with four evaluation strategies (fine-tuned classifier, separate evaluator, masked retraining
    % with positional embeddings,
    and masked retraining without positional embeddings) on the ViT-Base architecture.
    % evaluated with and without model retraining.
    \textbf{Left:} inserting features from
    % in order of
    most to least important.
    \textbf{Right:} removing features from
    % in order of
    most to least important.
    }
    \label{fig:roar_all}
    % \vskip -0.2cm
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/roar_imagenette.tex <==
\begin{figure}[t]
    %\vspace{-.2cm}
    % \vspace{.5cm}
    \vskip -0.1in
    \figurespacing
    \centering
    %\includegraphics[width=0.94\linewidth]{images/roar_imagenette.pdf}
    \includegraphics[width=0.95\linewidth]{images/roar_imagenette_all_delete.pdf}
    \caption{ImageNette accuracy when removing features in order of
    % according to
    their importance, run with four evaluation strategies: fine-tuned classifier, separate evaluator, masked retraining, and masked retraining without positional embeddings. 
    % (surrogate, separate evaluator and masked retraining).
    % evaluated with and without model retraining.
    % \textbf{Left:} inserting features from
    % % in order of
    % most to least important.
    % \textbf{Right:} removing features from
    % % in order of
    % most to least important.
    }
    \label{fig:roar}
    \vskip -0.2cm
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/roar_positional.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/roar_positional.pdf}
    \caption{
    ROAR evaluation with masked retraining, with and without positional embeddings in the retrained ViT. 
    }
    \label{fig:roar_positional}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/roar_vitsmall.tex <==
\begin{figure}[t]
    % \vspace{-.2cm}
    \figurespacing
    \centering
    \includegraphics[width=\linewidth]{images/roar_vitsmall.pdf}
    \caption{ImageNette accuracy when removing features in order of
    % according to
    their importance, run with four evaluation strategies (fine-tuned classifier, separate evaluator, masked retraining
    % with positional embeddings,
    and masked retraining without positional embeddings) on the ViT-Small architecture.
    % evaluated with and without model retraining.
    \textbf{Left:} inserting features from
    % in order of
    most to least important.
    \textbf{Right:} removing features from
    % in order of
    most to least important.
    }
    \label{fig:roar_vitsmall}
    \vspace{-.2cm}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/sensitivity.tex <==
\begin{figure}[t]
    % \vspace{-.2cm}
    \figurespacing
    \centering
    \includegraphics[width=0.95\linewidth]{images/sensitivity.pdf}
    \vskip -0.2cm
    \caption{
    Sensitivity-n evaluation
    for different subset sizes. The metric is generated separately for a range of subset sizes,
    whereas faithfulness is calculated jointly over subsets of all sizes.
    }
    \label{fig:sensitivity}
    \vskip -0.3cm
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/sensitivity_nontarget.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{images/sensitivity_nontarget.pdf}
    \caption{
    Sensitivity-n evaluation for non-target classes. The results are generated separately for each subset size and averaged across all non-target classes.
    }
    \label{fig:sensitivity_nontarget}
\end{figure}

==> ViT Shapley (ICLR 2023)/figures/times.tex <==
\begin{table}[t]
\centering
\caption{
Time to generate explanations for a single sample (in milliseconds). For class-specific explanations, the running time involves generating explanations for all classes.
} \label{tab:times}
\vskip 0.1in
\begin{center}
\begin{small}
% \begin{scriptsize}
% {\tablesize
    \begin{tabular}{lrrr}
    \toprule
     & ImageNette & MURA & Pets\\
    \midrule
    Attention last & 6.8 & 6.4 & 6.2\\
    Attention rollout & 10.6 & 10.0 & 11.1\\\midrule
    GradCAM & 275.9 & 26.2 & 986.4 \\
    IntGrad & 1236.8 & 123.3 & 5004.9 \\
    Vanilla & 230.1 & 23.0 & 810.7 \\
    SmoothGrad & 1218.0 & 121.2 & 4854.8 \\
    VarGrad & 1218.9 & 121.3 & 4882.5 \\
    LRP & 1551.4 & 155.7 & 5583.5 \\\midrule
    Leave-one-out & 810.0 & 815.9 & 922.5 \\
    RISE & 8213.4 & 8171.1 & 8919.8 \\
    \textbf{ViT Shapley} & 10.1 & 10.2 & 10.8 \\
    \bottomrule
    \end{tabular}
% }
% \end{scriptsize}
\end{small}
\end{center}
\end{table}

==> ViT Shapley (ICLR 2023)/preamble/definitions.tex <==
% THEOREMS
\newtheorem{prop}{Proposition}
\newtheorem{thmdef}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{corr}{Corollary}
\newtheorem{thm}{Theorem}
\newtheorem{appthm}{Theorem}
\newtheorem{asmp}{Assumption}

% COUNTERS
\renewcommand{\labelenumi}{\color{black!67}{\arabic{enumi}.}}
\renewcommand{\labelenumii}{{\color{black!67}(\alph{enumii})}}
\renewcommand{\labelitemi}{{\color{black!67}\textbullet}}

\crefname{thmdef}{definition}{definitions}
\crefname{lemma}{lemma}{lemmas}
\crefname{prop}{proposition}{propositions}
\crefname{algorithm}{algorithm}{algorithms}

% COMMENTS
\newif\ifprintcomments
\newcommand{\authorcomment}[3]{
	\ifprintcomments
		{\bf \color{#1} (#2: #3)}
	\else
		{}
	\fi
}

% COLORS
\definecolor{deepblue}{HTML}{20639B}
\definecolor{seagreen}{HTML}{3CAEA3}
\definecolor{niceyellow}{HTML}{D19654}
\definecolor{nicegreen}{HTML}{6a040f}
\definecolor{niceblue}{HTML}{277DA1}

% ALGORITHM
\newlength\myindent
\setlength\myindent{2em}
\newcommand\bindent{%
    \begingroup
    \setlength{\itemindent}{\myindent}
    \addtolength{\algorithmicindent}{\myindent}
}
\newcommand\eindent{\endgroup}

% TREES
\forestset{
    .style={
        for tree={
            base=bottom,
            child anchor=north,
            align=center,
            s sep+=1cm,
    straight edge/.style={
        edge path={\noexpand\path[\forestoption{edge},thick,-{Latex}] 
        (!u.parent anchor) -- (.child anchor);}
    },
    if n children={0}
        {tier=word, draw, thick, rectangle}
        {draw, diamond, thick, aspect=2},
    if n=1{%
        edge path={\noexpand\path[\forestoption{edge},thick,-{Latex}] 
        (!u.parent anchor) -| (.child anchor) node[pos=.2, above] {Y};}
        }{
        edge path={\noexpand\path[\forestoption{edge},thick,-{Latex}] 
        (!u.parent anchor) -| (.child anchor) node[pos=.2, above] {N};}
        }
        }
    }
}

%FOOTNOTES
\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother

% Random additions
\newcommand\tablesize{\fontsize{8pt}{10pt}\selectfont}
\newcommand\figurespacing{\vspace{-0.7cm}}

==> ViT Shapley (ICLR 2023)/preamble/math.tex <==
% This file is for new math commands only.
% NO IMPORT STATEMENTS

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\seCref#1{section~\ref{#1}}
% Section reference, capital.
\def\SeCref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twoseCrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\seCrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvxt{{\widetilde{\mathbf{x}}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution


\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


% EDIT BELOW THIS POINT ---------
\newcommand{\E}{\mathbb{E}}
% \newcommand{\phifast}{\phi_{\text{fast}}}
\newcommand{\phifast}{\phi_{\text{ViT}}}
% \newcommand{\phifast}{\phi_{\text{vt}}}
\newcommand{\inv}{^{-1}}
\newcommand{\psh}{p_{\text{Sh}}}
% \newcommand{\hin}{h_{in}}
% \newcommand{\hout}{h_{out}}
\newcommand{\hin}{h}
\newcommand{\hout}{h'}
\newcommand{\rvQ}{\mathbf{Q}}
\newcommand{\rvK}{\mathbf{K}}
\newcommand{\rvV}{\mathbf{V}}
\newcommand{\rvA}{\mathbf{A}}
\newcommand{\rvS}{\mathbf{S}}


==> ViT Shapley (ICLR 2023)/preamble/packages.tex <==
% ####### PACKAGES ONLY

\usepackage{amssymb, amsmath, amsthm}
\usepackage{mathtools}
\usepackage{xcolor}


% SPACING and TEXT

\usepackage{microtype}
\usepackage[english]{babel}
\usepackage[parfill]{parskip}
\usepackage{enumitem}
\usepackage{wrapfig}
\usepackage{multicol}
\usepackage{float}
\usepackage{adjustbox}
\usepackage[utf8]{inputenc} % allow utf-8 input

% FONTS
% fontenc needed for small caps
\usepackage[T1]{fontenc}
\usepackage{amsfonts}
\usepackage{bm}
\usepackage{bbm}
\usepackage{times}

% HEADER AND FOOTER
\usepackage{fancyhdr}

% FIGURES
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{subcaption}
\usepackage{tikz}
\usepackage{forest}
\usetikzlibrary{arrows.meta}


% TABLES
\usepackage{booktabs}
\usepackage{caption}

% ALGORITHMS
% \usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage[ruled,vlined]{algorithm2e}
\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}
\usepackage{listings}
\usepackage{fancyvrb}
\fvset{fontsize=\normalsize}

% % BIBLIOGRAPHY
% \usepackage[round]{natbib}
\renewcommand{\bibname}{References}
\renewcommand{\bibsection}{\subsubsection*{\bibname}}

% If you use BibTeX in apalike style, activate the following line:
\bibliographystyle{apalike}

% ACRONYMS
\usepackage[acronym,smallcaps,nowarn]{glossaries}
\glsdisablehyper
% \makeglossaries

% HYPERREF
% \usepackage[colorlinks=true,linktoc=all]{hyperref}
\usepackage[linktoc=all]{hyperref}
\usepackage[all]{hypcap}
% \hypersetup{citecolor=deepblue}
% \hypersetup{citecolor=black}
% \hypersetup{linkcolor=deepblue}
\hypersetup{linkcolor=black}
% \hypersetup{urlcolor=magenta}


% URL
\usepackage{url}
\usepackage[nameinlink]{cleveref}

% COLUMNS
\usepackage{multirow}
\setlength{\columnsep}{0.5cm}

% FUN
\usepackage{nicefrac}
% \usepackage{todonotes}

% FLEXIBLE FOOTNOTES
% \usepackage[symbol]{footmisc}
% \renewcommand{\thefootnote}{\fnsymbol{footnote}}

==> ViT Shapley (ICLR 2023)/sections/abstract.tex <==
\begin{abstract}
    Transformers have become a default architecture in computer vision, but understanding what drives their predictions remains a challenging problem. Current explanation approaches rely on attention values or input gradients, but these provide a limited view
    % only a limited understanding
    of a model's dependencies.
    Shapley values offer a theoretically sound alternative, but their computational cost makes them impractical for large, high-dimensional models.
    In this work, we aim to make Shapley values practical for vision transformers (ViTs). To do so, we first leverage an attention masking approach to evaluate ViTs with partial information, and we then
    % develop a learning-based approach that generates Shapley value explanations as efficiently as the original predictions.
    % train a separate explainer model that generates Shapley value explanations as efficiently as the original predictions.
    % develop an approach to train a separate explainer model that generates efficient Shapley value explanations.
    develop a procedure to generate
    % for generating
    Shapley value explanations via a
    separate, learned
    % separately trained
    % separate, learned
    explainer model.
    % for estimating Shapley values
    % Shapley value approximation
    % estimation approach
    % that generates explanations
    % lets us generate explanations
    % We develop a learning-based Shapley value estimation approach that involves fine-tuning a pre-trained ViT, and this allows us to generate explanations
    % thereby enabling explanations that are generated
    % We conduct experiments comparing Shapley values to many
    Our experiments compare Shapley values to many
    % a large number of
    baseline
    % existing
    methods (e.g., attention rollout, GradCAM, LRP), and we find that our approach provides more accurate explanations than
    % many existing methods
    % any
    % previously available
    existing
    methods
    for ViTs.
\end{abstract}

==> ViT Shapley (ICLR 2023)/sections/background.tex <==
Here, we define notation used throughout the paper and briefly introduce Shapley values.

\subsection{Notation}

Our focus is vision transformers trained for classification tasks, where $\rvx \in \R^{224 \times 224 \times 3}$ denotes an image and $\rvy \in \{1, \ldots, K\}$ denotes the class. We write the image patches as $\rvx = (\rvx_1, \ldots, \rvx_d)$, where ViTs typically have $\rvx_i \in \R^{16 \times 16 \times 3}$ and $d = 196$. The model is given by $f(\rvx; \eta) \in [0, 1]^K$ and $f_y(\rvx; \eta) \in [0, 1]$ represents the probability for the $y$th class. Shapley values involve feature subsets, so we use $s \in \{0, 1\}^d$ to denote a subset of indices and $\rvx_s = \{\rvx_i : s_i = 1\}$ a subset of image patches. We also use $\vzero$ and $\vone \in \R^d$ to denote vectors of zeros and ones, and $e_i \in \R^d$ is a vector with a one in the $i$th position and zeros elsewhere. Finally, bold symbols $\rvx, \rvy$ are random variables, $x, y$ are possible values, and $p(\rvx, \rvy)$ denotes the data distribution.

% \subsection{Notation}

% Given a classifier $f(\rvx; \eta)$, we let $f_y(\rvx; \eta) \in [0, 1]$ denote the prediction probability for the $y$th class, where $y \in \{1, \ldots, K\}$. We denote the various input features as $\rvx_1, \ldots, \rvx_d$, where for vision transformers each $\rvx_i$ is an image patch, so that $\rvx_i \in \R^{16 \times 16 \times 3}$ and $d = 196$. We let $s \in \{0, 1\}^d$ represent subsets of indices and $\rvx_s = \{\rvx_i : i \in s\}$ subsets of features, and we use $\vzero \in \R^d$ and $\vone \in \R^d$ to denote vectors of zeros and ones, so that $\vone^\top s$ is the cardinality of $s$.

% TODO revise this (missing $e_i$, RVs vs. values)

\subsection{Shapley values}

Shapley values were developed in game theory for allocating
credit in coalitional games \citep{shapley1953value}. A coalitional game is represented by a set function, and the value for each subset indicates the profit achieved when the corresponding players participate. Given a game with $d$ players, or a set function $v: \{0, 1\}^d \mapsto \R$, the Shapley values are denoted by $\phi_1(v), \ldots, \phi_d(v) \in \R$ for each player, and the value $\phi_i(v)$ for the $i$th player is defined as follows:
\begin{equation}
    \phi_i(v) = \frac{1}{d} \sum_{s : s_i = 0} \binom{d - 1}{\vone^\top s}\inv \big( v(s + e_i) - v(s) \big). \label{eq:shapley}
\end{equation}
Intuitively, \cref{eq:shapley} represents the change in profit from introducing the $i$th player, averaged across all possible subsets to which $i$ can be added. Shapley values are defined in this way to satisfy many reasonable properties: for example, the credits sum to the value when all players participate, players with equivalent contributions receive equal credit, and players with no contribution receive zero credit \citep{shapley1953value}. These properties make Shapley values attractive in many settings: they have been applied with coalitional games that represent a model's prediction given a subset of features (SHAP) \citep{vstrumbelj2010efficient, lundberg2017unified}, as well as several other use-cases in machine learning \citep{ghorbani2019data, ghorbani2020neuron, covert2020understanding}.

There are two main challenges when using Shapley values to explain individual predictions \citep{chen2022algorithms}. The first is properly withholding feature information, and we explore how to address this challenge in the ViT context (\Cref{sec:removal}). The second is calculating Shapley values efficiently, because their computation scales exponentially with the number of inputs $d$. Traditionally, they are approximated using sampling-based estimators like KernelSHAP \citep{castro2009polynomial, vstrumbelj2010efficient, lundberg2017unified}, but we build on a more efficient learning-based approach (FastSHAP) recently introduced by \cite{jethani2021fastshap} (\Cref{sec:estimation}).

==> ViT Shapley (ICLR 2023)/sections/conclusion.tex <==
In this work, we developed a learning-based approach to generate Shapley values for ViTs.
% vision transformers.
Our approach involves training a separate explainer model
using an objective that does not require ground truth supervision,
% using a loss function that circumvents the need for ground truth Shapley values,
and ViT Shapley outperforms a variety of attention- and gradient-based methods across a range of
accuracy
metrics.
Our experiments provide empirical support
% evidence for the potential
for Shapley values as an alternative to attention-based approaches, which remain popular for transformer models.
Future directions involve extending ViT Shapley to NLP models,
% transformer models in NLP,
operating with arbitrary token groups or superpixels, and accelerating or otherwise improving the explainer model's training.

==> ViT Shapley (ICLR 2023)/sections/estimation.tex <==
Given our approach for evaluating ViTs with partial information, we can use Shapley values to identify influential image patches for an input $x$ and class $y$. This involves evaluating the model with many feature subsets $x_s$, so we define a coalitional game $v_{xy}(s) = g_y(x_s; \beta)$. Alternatively, if we use a model trained with masking, we can define the coalitional game as $v_{xy}(s) = f_y(x_s; \eta)$.
% Standard
Common Shapley value approximations are based on sampling feature permutations \citep{castro2009polynomial, vstrumbelj2010efficient} or fitting a weighted least squares model \citep{lundberg2017unified, covert2021improving}, but these can require hundreds or thousands of model evaluations to explain a single prediction.\footnote{The number of model evaluations depends on how fast the estimators converge, and we find that KernelSHAP requires >100,000 samples to converge for ViTs (\Cref{app:results}).} Instead, we develop a learning-based estimation approach for ViTs.

Our goal is to obtain an explainer model that estimates Shapley values directly. To do so, we train a new vision transformer $\phifast(\rvx, \rvy; \theta) \in \R^d$ that outputs approximate Shapley values for an input-output pair $(x, y)$ in a single forward pass. Crucially, rather than training the model using a dataset of ground truth Shapley value explanations, we train it by minimizing the following objective,

\vskip -0.15in
\begin{align}
    \mathcal{L}(\theta) =\; &\E_{p(\rvx, \rvy)}
    \E_{\psh(\rvs)} \Big[ \big( v_{\rvx \rvy}(\rvs) - v_{\rvx \rvy}(\vzero) - \rvs^\top \phifast(\rvx, \rvy; \theta) \big)^2 \Big] \label{eq:objective} \\
    &\text{s.t.} \quad \vone^\top \phifast(x, y; \theta) = v_{x y}(\vone) - v_{x y}(\vzero) \quad \forall \; (x, y), \nonumber
\end{align}
% \vskip -0.1in

where $\psh(\rvs)$ is a distribution defined as $\psh(s) \propto (\vone^\top s - 1)!(d - \vone^\top s - 1)!$ for $0 < \vone^\top s < d$ and $\psh(\vone) = \psh(\vzero) = 0$. Intuitively, \cref{eq:objective} encourages the explainer model to output feature scores that provide an additive approximation for the predictions with partial information, where the predictions are represented by $v_{\rvx\rvy}(\rvs)$ and the additive approximation by $v_{\rvx \rvy}(\vzero) + \rvs^\top \phifast(\rvx, \rvy; \theta)$.

% TODO trying out removing this part
% This loss function is derived from an optimization-based characterization of the Shapley value,
% % that views it as
% which states that it is
% the solution to a specific weighted least squares problem \citep{charnes1988extremal}.
% % the Shapley value's weighted least squares characterization \citep{charnes1988extremal}, which states that the Shapley values are the optimal coefficients in a specific weighted least squares problem.
% % The loss function
% It was recently introduced by Jethani et al. \citep{jethani2021fastshap},
% % This loss function is derived from the Shapley value's weighted least squares characterization \citep{charnes1988extremal} and was introduced by Jethani et al. \citep{jethani2021fastshap},
% % The loss function is derived from the Shapley value's characterization as the solution to a weighted least squares problem \citep{charnes1988extremal},
% and it satisfies the property that its global optimizer $\phifast(\rvx, \rvy; \theta^*)$
% % is a function that
% outputs the exact Shapley values, or
% $\phifast(x, y; \theta^*) = \phi(v_{x y})$
% % $\phifast(\rvx, \rvy; \theta^*) = \phi(v_{\rvx \rvy})$
% % almost everywhere in $p(\rvx, \rvy)$
% (see proof in \citep{jethani2021fastshap}).

%%%%%%%%%%
% TODO insert new theoretical results here

The loss in \cref{eq:objective} was introduced by \cite{jethani2021fastshap} and is derived from an optimization-based characterization of the Shapley value \citep{charnes1988extremal}.
% which states that it is the solution to a specific weighted least squares problem \citep{charnes1988extremal}.
% To further
To rigorously justify this
% explainer model
training approach, we derive
% introduce
new results that show how this objective
% our loss function
controls
% linking this loss function to
the Shapley value estimation error.
% (see proofs in \Cref{app:proofs}).
% , or the distance between the exact and approximated Shapley values.
Proofs
% for our results
are
% provided
in \Cref{app:proofs}.
First, we show that the explainer's
% expected
loss for a single input is strongly convex in the prediction, a result that implies the existence of unique optimal predictions.
% a result that helps reason about the optimal predictions \citep{gneiting2007strictly}.

\begin{lemma} \label{lemma1}
For a single input-output pair $(x, y)$,
% with prediction $\phi = \phifast(x, y; \theta)$,
% under our objective function (\cref{eq:objective}),
% Under our objective function in \cref{eq:objective},
the expected loss under \cref{eq:objective} for the prediction
% $\phi = \phifast(x, y; \theta)$
$\phifast(x, y; \theta)$
% is a $\mu$-strongly convex function $h_{xy}(\phi)$
is $\mu$-strongly convex
% of $\phi$
with $\mu = H_{d - 1}\inv$, where $H_{d - 1}$ is the $(d - 1)$th harmonic number.
\end{lemma}

Next, we utilize the strong convexity property from \Cref{lemma1} to prove our main result: that the explainer model's loss function upper bounds the distance between the exact and approximated
% approximated and exact
Shapley values.
% even though
This is notable because we do not utilize ground truth values during training.
% we cannot access these during training.

\begin{thm} \label{theorem1}
For a model $\phifast(\rvx, \rvy; \theta)$ whose predictions satisfy the constraint in \cref{eq:objective}, the objective value $\mathcal{L}(\theta)$ upper bounds the Shapley value estimation error as follows,
% expected distance to the exact Shapley values,
\begin{equation*}
    \E_{p(\rvx, \rvy)} \Big[ \big|\big|\phifast(\rvx, \rvy; \theta) - \phi(v_{\rvx \rvy})\big|\big|_2 \Big]
    \leq \sqrt{2 H_{d - 1} \Big( \mathcal{L}(\theta) - \mathcal{L}^* \Big)},
\end{equation*}
where $\mathcal{L}^*$ represents the loss achieved by the exact Shapley values.
\end{thm}

%%%% Without corollary included

This shows that our objective is a viable approach for training without exact Shapley values, because optimizing \cref{eq:objective} minimizes an upper bound on the estimation error.
% Finally, we show that this implies convergence to the exact Shapley values in the limit that the loss approaches its optimum.
In other words, if we can iteratively optimize the explainer model so that its loss approaches the optimum obtained by the exact Shapley values ($\mathcal{L}(\theta) \to \mathcal{L}^*$), our estimation error will go to zero.

%%%% With corollary included

% This shows that our objective
% % function
% is a viable approach for training without
% % alternative to
% % substitute for
% % training with
% exact Shapley values,
% % as ground truth labels,
% because optimizing \cref{eq:objective}
% % our loss
% % the loss
% % is equivalent to minimizing
% minimizes
% % minimizes
% an upper bound on the estimation error. Finally, we show that this
% % \Cref{theorem1}
% implies convergence to the exact Shapley values in the limit that the loss approaches its optimum.
% % in the optimal-model limit.
% % This coincides with the claim from Jethani et al. \citep{jethani2021fastshap} that the globally optimal explainer outputs exact Shapley values.

% \begin{corr} \label{corollary1}
% Given a sequence of models $\phifast(\rvx, \rvy; \theta_1), \phifast(\rvx, \rvy; \theta_2), \ldots$
% % $\phifast(\rvx, \rvy; \theta_n)$ for $n = 1, \ldots$
% % $\theta_1, \theta_2, \ldots$
% % for $n = 1, \ldots$,
% whose predictions
% % $\phifast(\rvx, \rvy; \theta_n)$
% satisfy the constraint in \cref{eq:objective} and where
% % with
% $\mathcal{L}(\theta_n) \to \mathcal{L}^*$,
% % \begin{equation*}
% %     \lim_{n \to \infty} \mathcal{L}(\theta_n) = \mathcal{L}^*,
% % \end{equation*}
% the Shapley value estimation error
% % expected distance to the Shapley values
% % tends
% goes to zero:
% \begin{equation*}
%     \lim_{n \to \infty} \E_{p(\rvx, \rvy)} \Big[ \big|\big|\phifast(\rvx, \rvy; \theta_n) - \phi(v_{\rvx \rvy})\big|\big|_2 \Big] = 0.
% \end{equation*}
% \end{corr}
% This shows that if we can iteratively optimize the explainer model such that its loss approaches the optimum obtained by the exact Shapley values, our estimation error goes to zero.

%%%%

%%%%%%%%%%

\input{figures/qualitative}

In practice, we train the explainer model $\phifast(\rvx, \rvy; \theta)$ using stochastic gradient descent, and several other steps are important during training. First, we normalize the explainer's unconstrained predictions in order to satisfy the objective's constraint in \cref{eq:objective}; this ensures that the Shapley value's \textit{efficiency} property holds \citep{shapley1953value}. Next, rather than training the explainer from scratch, we fine-tune an existing model that can be either the original classifier or a ViT pre-trained on a different supervised or self-supervised learning task \citep{touvron2021training, he2021masked}; ViTs are more difficult to train than convolutional networks, and we find that fine-tuning is important to train the explainer effectively (\Cref{tab:ablations}).
% We can use the original classifier as an initialization, or we can use a ViT pre-trained on a different supervised or self-supervised learning task \citep{touvron2021training, he2021masked}. 
Finally, we simplify the architecture by estimating Shapley values for all classes simultaneously. Our training approach is described in more detail in \Cref{app:method}.

By using a ViT to estimate Shapley values, we model the true explanation function and learn rich representations that capture not only which class is represented, but where key information is located.
% By using a ViT to estimate Shapley values, we leverage the model's internal representation to produce similar explanations for similar inputs.
And by fine-tuning an existing model, we allow the explainer to re-use visual features that were informative for other challenging tasks.
% (\Cref{app:method}, \Cref{tab:ablations}).
Ultimately, the explainer cannot guarantee exact Shapley values, but no approximation algorithm can; instead, it offers a favorable trade-off between accuracy and efficiency, and we find empirically that this approach offers a powerful alternative to the methods currently used for ViTs.


==> ViT Shapley (ICLR 2023)/sections/experiments.tex <==
We now demonstrate the effectiveness of our approach, termed \textit{ViT Shapley}.\footnote{\url{https://github.com/suinleelab/vit-shapley}}
% \footnote{Code to be released upon publication.}
% \footnote{\url{https://github.com/suinleelab/vit-shapley}}
First, we evaluate attention masking for handling held-out patches in ViTs (\Cref{sec:removal_metrics}). Next, we compare explanations from ViT Shapley to several existing methods (\Cref{sec:explanation_metrics}). Our baselines include attention-, gradient- and removal-based explanations, and we compare these methods via several metrics for explanation quality, including insertion/deletion of important features \citep{petsiuk2018rise},
sensitivity-n \citep{ancona2018towards}, faithfulness \citep{bhatt2021evaluating} and ROAR \citep{hooker2019benchmark}.

Our experiments are based on three image datasets: ImageNette, a natural image dataset consisting of ten ImageNet classes \citep{howard2020fastai, deng2009imagenet}, MURA, a medical image dataset of musculoskeletal radiographs classified as normal or abnormal \citep{rajpurkar2017mura}, and the Oxford IIIT-Pets dataset, which has 37 classes \citep{parkhi2012cats}. See \Cref{fig:qualitative} for example images. 
The main text shows results for ImageNette and MURA,
% ImageNette and MURA results are shown in the main text,
% Our main text results focus on ImageNette and MURA,
and Pets results are in \Cref{app:results}.
% results for the Pets dataset are in \Cref{app:results}.
% ImageNette contains 13,394 examples and ten classes, and MURA contains 40,005 examples and two classes; see \Cref{fig:qualitative} for examples from each dataset.
We use ViT-Base models \citep{rw2019timm} as classifiers for all datasets, unless otherwise specified.

\subsection{Evaluating image patch removal} \label{sec:removal_metrics}

Our initial experiments test whether attention masking is effective for handling held-out image patches. We fine-tuned the classifiers for each dataset
% both datasets
following the procedure described in \Cref{sec:removal}, and we also tested several approaches without performing any fine-tuning: attention masking, attention masking applied after the softmax operation (how dropout is often implemented for ViTs, \citealt{rw2019timm}), setting input patches to zero \citep{naseer2021intriguing}, setting token embeddings to zero, and replacing with random patches from the dataset. Finally, we performed identical fine-tuning while replacing input patches with zeros, which is equivalent to introducing a fixed mask token.

As a measure of how well missing patches are handled, we calculated the KL divergence relative to the full-image predictions as random patches are removed. This can be interpreted as a divergence measure between the masked predictions and the predictions with patches marginalized out (see \Cref{app:masked_training}), or how close we are to correctly removing patch information. The metric is calculated
% on the test set
with randomly generated patch subsets, and it represents whether the model makes reasonable predictions given partial inputs. Similar results for top-1 accuracy are in \Cref{app:results}.

\input{figures/removal}

\Cref{fig:removal} shows the results. Most methods perform well with $<$25\% of patches missing, leading to only small increases in KL divergence. This is especially true for ImageNette, where large objects make the model more robust to missing patches. However, the methods with no fine-tuning begin to diverge as larger numbers of patches are removed and the partial inputs become increasingly off-manifold.
Thus, fine-tuning becomes necessary to properly account for partial inputs
% avoid poor performance
as more patches are removed.

For all datasets, we find that fine-tuning with either attention masking or input patches set to zero provide comparable performance, and that these perform best across all numbers of patches. This means that fine-tuning makes attention masking significantly more effective for marginalizing out missing patches, and these results suggest that training ViTs with held-out tokens may be necessary to enable robustness to partial information. As prior work suggests, properly handling held-out information is crucial for generating informative explanations \citep{frye2020shapley, covert2021explaining}, so the remainder of our experiments proceed with the fine-tuned attention masking approach.

\subsection{Evaluating explanation accuracy} \label{sec:explanation_metrics}

Next, we implemented ViT Shapley by training explainer models for both datasets. We used the fine-tuned classifiers from \Cref{sec:removal_metrics} to handle partial information, and we used the ViT-Base architecture with extra output layers to generate Shapley values for all patches. The explainer models were trained by optimizing \cref{eq:objective} using stochastic gradient descent (see details in \Cref{app:method}), and once trained, the explainer outputs approximate Shapley values in a single forward pass (\Cref{fig:qualitative}).

As comparisons for ViT Shapley, we considered
% many baseline methods.
a large number of baselines.
For attention-based methods, we use attention rollout and the last layer's attention directed to the class token \citep{abnar2020quantifying}. Similar to prior work \citep{chefer2021transformer}, we did not use attention flow due to the computational cost. Next, for gradient-based methods, we use Vanilla Gradients \citep{simonyan2013deep},
% Integrated Gradients
IntGrad \citep{sundararajan2017axiomatic}, SmoothGrad \citep{smilkov2017smoothgrad}, VarGrad \citep{hooker2019benchmark}, LRP \citep{chefer2021transformer} and GradCAM \citep{selvaraju2017grad}.
% We used existing LRP and GradCAM implementations for ViTs \citep{chefer2021transformer}, and the remaining gradient-based methods were run using the Captum package \citep{kokhlikyan2020captum}.
% Finally,
For removal-based methods, we use the leave-one-out approach \citep{zeiler2014visualizing} and RISE \citep{petsiuk2018rise}.
% , which we implemented from scratch.
\Cref{app:baselines} describes the baselines in more detail, including how several
% methods
were modified to provide patch-level results, and \Cref{app:results} shows the running time for each method.

Given our set of baselines, we used several metrics to evaluate ViT Shapley. Evaluating explanation accuracy is difficult when the true importance is not known a priori, so we rely on metrics that test how removing (un)important features affects a model's predictions. Intuitively, removing influential features for a particular class should reduce the class probability, and removing non-influential features should not affect or even increase the class probability. Removal-based explanations are implicitly related to such metrics \citep{covert2021explaining}, but attention- and gradient-based methods may be hoped to provide strong performance with lower computational cost.

\input{figures/metrics}

First, we implemented the widely used \textit{insertion} and \textit{deletion} metrics \citep{petsiuk2018rise}. For these, we generate predictions while inserting/removing features in order of most to least important, and we then evaluate the area under the curve of prediction probabilities (see \Cref{fig:qualitative}). Here, we average the results across 1,000 images for their true class. We use random test set images for ImageNette, and for MURA we use test examples that were classified as abnormal because these are more important in practice. When removing information, we use the fine-tuned classifier because this represents the closest approximation to properly
% truly
removing information from the model (\Cref{sec:removal}).

\Cref{tab:metrics} displays the results, and we find that ViT Shapley offers the best performance on both datasets. RISE and LRP tend to be the most competitive baselines, and perhaps surprisingly, certain other methods fail to outperform a random baseline (GradCAM, SmoothGrad, VarGrad). The baselines are sometimes competitive with ViT Shapley on insertion, but the gap for the deletion metric is larger. Practically, this means that ViT Shapley identifies important features that quickly drive the prediction towards a given class, and that quickly reduce the prediction probability when deleted.

\input{figures/metrics_nontarget}

Next, we modified these metrics to address a common issue with model explanations: that their results are not specific to each class \citep{rudin2019stop}. ViT Shapley produces separate explanations for each class, so it can identify relevant patches even for non-target classes (see \Cref{fig:qualitative}). \Cref{tab:metrics_nontarget} shows insertion/deletion results averaged across all non-target classes for ImageNette. The attention-based methods do not produce class-specific explanations, and the remaining baselines generally provide poor results. Empirically, this is because the explanations are often similar across classes (see \Cref{app:qualitative}). ViT Shapley performs best, particularly on insertion, and RISE is the best-performing baseline. \Cref{app:results} shows results for MURA, as well as the curves used to calculate these results.

% Insertion and deletion
The insertion and deletion metrics
only test importance rankings, so we require other
metrics
to test the specific attribution values. \textit{Sensitivity-n} \citep{ancona2018towards} was proposed for this purpose, and it measures
% as a way to measure
whether attributions correlate with the impact on a model's prediction when a feature is removed. The correlation is
% often
typically
calculated
across
% random
subsets of a fixed size, and then averaged across many predictions.
% Similarly,
\textit{Faithfulness} \citep{bhatt2021evaluating} is a similar
% related
% nearly identical
metric where the correlation is calculated
% only once
across subsets of all sizes.

\Cref{tab:metrics} and \Cref{tab:metrics_nontarget} show faithfulness results.
% and we observe that ViT Shapley performs best for both target and non-target class explanations.
Among the baselines, RISE and LRP remain most competitive, but ViT Shapley again performs best for both datasets.
% target and non-target class explanations.
\Cref{fig:sensitivity} shows sensitivity-n results calculated across a range of subset sizes.
% ViT Shapley again performs the best overall, particularly for smaller subsets, and
Leave-one-out naturally performs best for large subset sizes, but ViT Shapley
% again
performs the best overall, particularly with smaller subsets.
The sensitivity-n results focus on the target class,
but \Cref{app:results} shows
results for non-target classes where ViT Shapley's advantage over many baselines (including LRP) is even larger.

\input{figures/sensitivity}

Finally, we performed an evaluation inspired by ROAR \citep{hooker2019benchmark}, which tests how a model's accuracy degrades as important features are removed. ROAR suggests retraining
% the model
with masked inputs, but this is
% arguably
unnecessary here
% in our case
because the fine-tuned classifier is designed to handle
% surrogate handles
held-out patches. We therefore generated multiple versions of the metric. First, we evaluated accuracy while using the fine-tuned classifier to handle masked patches. Second, we
% recalculated the metric
repeated the evaluation
using a separate evaluator model trained directly with held-out patches,
% (see \Cref{sec:removal}),
similar to EVAL-X \citep{jethani2021have}. Third, we performed masked retraining as described by ROAR. The first version represents the original classifier's best-effort prediction, and the second is a best-effort prediction disconnected from the original model; masked retraining is similar, but the retrained model can exploit information communicated by the masking, such as the shape and position of the removed object.

\input{figures/roar_imagenette}

\Cref{fig:roar} shows the results when removing important patches.
ViT Shapley consistently outperforms the baselines across the first two versions of the metric, yielding
faster degradation when important patches are removed. ViT Shapley also performs best when inserting important patches, yielding a faster increase in accuracy
(\Cref{app:results}).
It is outperformed by several baselines
with masked retraining
in the deletion direction (\Cref{fig:roar} bottom left), but we find that this is likely
% suspect this is
due to spatial information leaked by
ViT Shapley's deleted patches;
indeed, when we retrained
\textit{without positional embeddings},
we found that ViT Shapley achieved the fastest degradation with a small number of deleted patches (\Cref{fig:roar} bottom right).
Interestingly, positional embeddings in ViTs
% within ViTs
offer a unique approach to alleviate
ROAR's known
information leakage issue
\citep{jethani2021have}.

% TODO mention all key supplementary results:
% - More architectures
% - Explaining model directly (no fine-tuning)
% - Pets results
% - KernelSHAP comparisons
% - Qualitative examples

In addition to these experiments, we include many further results in the supplement (\Cref{app:results}). First, we observe similar benefits for ViT Shapley when using the Oxford-IIIT Pets dataset. Next, regarding the choice of architecture, we observe consistent results when replacing ViT-Base with ViT-Tiny, -Small or -Large. We also replicate our results when using a classifier trained directly with random masking, an approach discussed in prior work to accommodate partial input information \citep{covert2021explaining}. We then generated metrics comparing ViT Shapley's approximation quality with KernelSHAP \citep{lundberg2017unified}, and we found that ViT Shapley's accuracy is equivalent to running KernelSHAP for roughly 120,000 model evaluations (\Cref{app:results}). Lastly, we provide qualitative examples in \Cref{app:qualitative}, including comparisons with the baselines.
% and with KernelSHAP.
Overall, these results show that ViT Shapley is a practical and effective approach for explaining ViT predictions.

% In addition to these experiments, we observed consistent results when replicating
% all metrics using ViT-Small
% and a ViT classifier trained directly with random masking
% (\Cref{app:results}).
% We also generated metrics comparing ViT Shapley's approximation quality with KernelSHAP \citep{lundberg2017unified}, and we found that ViT Shapley's accuracy is equivalent to running KernelSHAP for roughly 120,000 model evaluations (\Cref{app:results}).
% Lastly, we provide qualitative examples in \Cref{app:qualitative}, including
% % These include
% comparisons with the baselines and with KernelSHAP.
% Overall, these results show that ViT Shapley is a practical and effective approach
% % alternative to existing methods
% for explaining ViT
% % vision transformer
% predictions.


==> ViT Shapley (ICLR 2023)/sections/introduction.tex <==
% Hello world \cite{Lundberg2017}.

Transformers~\citep{vaswani2017attention} were originally introduced for NLP, but in recent years they
% were
have been
successfully adapted to a variety of other domains \citep{wang2020transformer, jumper2021highly}.
% \citep{wang2020transformer, huang2020tabtransformer, rives2021biological, jumper2021highly}.
% Tabular data, proteins, what else?
In computer vision, transformer-based models are now used for problems including image classification, object detection and semantic segmentation \citep{dosovitskiy2020image, touvron2021training, liu2021swin}, and they achieve state-of-the-art performance in many tasks \citep{wortsman2022model}.
% See ConvNext, Model Soups
The growing use of transformers in computer vision motivates the question of what drives their predictions:
% which inputs drive their predictions:
% how they generate predictions:
understanding a complex model's dependencies is an important problem in many applications,
% a central problem in explainable machine learning,
but the field has not settled on a solution for the transformer architecture.

Transformers are composed of alternating self-attention and fully-connected layers, where the self-attention operation associates attention
% weights
values
with every pair of tokens.
% pair-wise attention values to every two tokens.
In vision transformers (ViTs) \citep{dosovitskiy2020image}, the tokens represent non-overlapping image patches, typically a total of $14 \times 14 = 196$ patches each of size $16 \times 16$. It is intuitive to view
% An intuitive approach is to view
% attention as an
attention values as indicators
% attention as an indicator
% an indication
of feature importance \citep{abnar2020quantifying, ethayarajh2021attention},
% -- these values are automatically calculated during the forward pass, and at first glance they appear to make transformers inherently understandable to humans.
but
% however,
% analogizing transformer attention to human attention
interpreting transformer attention in this way
% manner
% as feature importance
is potentially misleading. Recent work has raised questions about
% disputed
the validity of attention as explanation \citep{serrano2019attention, jain2019attention, chefer2021transformer}, arguing that it provides an incomplete picture of
% only partially represents
a model's dependence on
% the features associated with
each token.
% \citep{kobayashi2020attention}.
% In a recent evaluation of attention-based explanations, they performed poorly on object localization metrics and

If attention is not a reliable indicator of feature importance, then what is? We consider the perspective that transformers
% In a sense,
% transformer models
are no
% not meaningfully
different from any other architecture,
% any other architecture,
and that we can explain their predictions using model-agnostic approaches
% methods
that are currently
% widely
used for other architectures.
% models.
% types.
% CNNs and/or tree ensembles.
Among these methods, Shapley values are a theoretically compelling approach
% in which
% where the
with feature importance scores
% values
that are designed to satisfy many desirable properties \citep{shapley1953value, lundberg2017unified}.

%%%%% Preprint version %%%%%
The main challenge for Shapley values in the transformer context is calculating them efficiently, because a naive calculation has exponential running time in the number of patches. If Shapley values are poorly approximated, they are unlikely to reflect a model's true dependencies, but calculating them with high
% to sufficient
accuracy is currently too slow to be practical. Thus, our work aims to make Shapley values practical for transformers, and for ViTs in particular. Our contributions include:

%%%%% Submission version %%%%%
% The main challenge for Shapley values in the transformer context is calculating them efficiently, because a naive calculation has
% % running time that is exponential
% exponential running time
% in the number of patches.
% % features.
% %  \citep{van2021tractability}.
% If Shapley values are poorly approximated, they are unlikely to reflect a model's true dependencies; however,
% % but
% calculating them to sufficient accuracy is currently too slow
% % using existing approximations \citep{castro2009polynomial, lundberg2017unified, covert2021improving} is too slow
% % may take too long
% to be practical.
% % useful in practice.
% Thus, our work aims to make Shapley values practical for transformers, and for vision transformers in particular.

% Our contributions include:
% % are:
% % the following:

\begin{enumerate}[leftmargin=20pt]
    \item We investigate several approaches for withholding input features from vision transformers, which is a key operation for computing Shapley values.
    % Shapley values involve
    % require a mechanism for
    % withholding features from the model, and we investigate several feature removal approaches specific to vision transformers.
    We find that ViTs can accommodate missing image patches by masking attention values
    % setting attention values to zero
    for held-out tokens,
    % but
    and
    that training
    % fine-tuning
    with random masking
    % dropping
    is important for models to
    % to help models
    properly handle
    % accommodate
    partial information.
    % improve the model's robustness to partial information.
    % find that vision transformers can accommodate missing features by zeroing attention values for held-out image patches.
    % investigate several approaches for doing so with transformers. Zeroing attention values for held-out tokens is a natural approach, but we find that fine-tuning the model is necessary to make vision transformers robust to missing image patches.
    \item We develop a learning-based approach to estimate Shapley values efficiently and accurately.
    % generate efficient and accurate Shapley value explanations.
    % that enables efficient and accurate Shapley value explanations.
    Our approach
    % is based on recent work and
    involves fine-tuning an existing ViT
    % architecture
    using a loss function designed specifically for Shapley values \citep{jethani2021fastshap}, and
    %  \citep{charnes1988extremal, jethani2021fastshap},
    % based on the Shapley value's weighted least squares characterization \citep{charnes1988extremal, jethani2021fastshap},
    % specialized loss function,
    % loss function motivated by the Shapley value's weighted least squares characterization,
    % and
    we prove that our loss bounds the
    % Shapley value
    estimation error without requiring ground truth values during training.
    Once trained,
    our explainer model
    % our approach
    % after being trained,
    % after training,
    % it
    provides a significant speedup over
    % relative to
    % improvement over
    % existing
    methods
    % approximations
    like
    % such as
    KernelSHAP \citep{lundberg2017unified}.
    % \citep{lundberg2017unified, covert2021improving}.
    % approaches.
    %%%%%
    % We also prove that our loss function bounds the Shapley value estimation error without requiring ground truth values during training.
    % TODO these descriptions sound lame. For someone not familiar with this work, it's not surprising or remarkable that our loss would control the estimation error. What's more surprising is that you can control it without having access to the exact values during training
    % We also derive a new theoretical result showing that our loss function bounds the Shapley value estimation error.
    % We also derive new results
    % % linking our loss function to the Shapley value estimation error.
    % to show that our loss function yields an upper bound on the Shapley value estimation error.
    % \item We derive new results to justify our explainer model's training approach; specifically, we show that the loss function introduced by Jethani et al. \citep{jethani2021fastshap} provides an upper bound on the Shapley value estimation error.
    %%%%%
    \item Our experiments compare the Shapley value-based approach to several groups of competing methods:
    % provide extensive comparisons between our Shapley value-based approach and several groups of competing approaches:
    attention-based, gradient-based and removal-based explanations. We find that our approach provides the best overall performance, correctly identifying influential and non-influential
    % highlighting influential
    patches for both target and non-target classes. We verify this using three image datasets,
    % use
    % one natural image dataset and one medical image dataset,
    and the results are consistent across multiple metrics.
    % These results are consistent across multiple metrics, and when using one natural image and one medical image dataset.
\end{enumerate}

Overall, our work shows that Shapley values can be made
% are
practical for vision transformers, and that they provide a compelling alternative to current attention- and gradient-based approaches.

==> ViT Shapley (ICLR 2023)/sections/related.tex <==
Understanding neural network predictions is a challenging problem that has been actively researched for the last decade \citep{simonyan2013deep, zeiler2014visualizing, ribeiro2016should}. 
We focus on \textit{feature attribution}, or identifying the specific input features that influence a prediction, but prior work has also considered other
problems \citep{olah2017feature, kim2018interpretability}.
The various techniques that have been developed can be grouped into several categories, which we describe below.

\paragraph{Attention-based explanations}
Transformers use self-attention to associate weights with each pair of tokens \citep{vaswani2017attention}, and a natural idea is to assess which tokens receive the most attention
% for a particular input
\citep{clark2019does, rogers2020primer, vig2020bertology}. There are several versions of this approach, including \textit{attention rollout} and \textit{attention flow}  \citep{abnar2020quantifying}, which analyze attention across multiple layers. Attention is a popular interpretation tool, but it is only one component in a sequence of nonlinear operations that provides an incomplete picture of a model's dependencies \citep{serrano2019attention, jain2019attention, wiegreffe2019attention}, and direct usage of attention weights
% it
has not been shown to perform well in vision tasks \citep{chefer2021transformer}.

\paragraph{Gradient-based methods}
For other deep learning models such as CNNs, gradient-based explanations are a popular family of approaches. There are many variations on the idea of calculating input gradients, including methods that modify the input (e.g., SmoothGrad, IntGrad) \citep{smilkov2017smoothgrad, sundararajan2017axiomatic, xu2020attribution}, operate at intermediate network layers (GradCAM) \citep{selvaraju2017grad}, or design modified backpropagation rules (e.g., LRP, DeepLift) \citep{bach2015pixel, shrikumar2016not, chefer2021transformer}. Although they are efficient to compute for arbitrary network architectures, gradient-based explanations achieve mixed results in quantitative benchmarks, including for object localization and the removal of influential features \citep{petsiuk2018rise, hooker2019benchmark, saporta2021benchmarking, jethani2021fastshap},
and they have been shown to be insensitive to the randomization of model parameters \citep{adebayo2018sanity}.

\paragraph{Removal-based explanations}
Finally, \textit{removal-based explanations} are those that quantify feature importance by explicitly withholding inputs from the model \citep{covert2021explaining}. For models that require all features to make predictions, several options for removing features include setting them to default values \citep{zeiler2014visualizing}, sampling replacement values \citep{agarwal2020explaining} and blurring images \citep{fong2017interpretable}. These methods work with any model type, but they tend to be slow because they require making many predictions. The simplest approach of removing individual features (known as \textit{leave-one-out}, \citealt{ethayarajh2021attention}) is relatively fast, but the computational cost increases as we examine more feature subsets.

Shapley values \citep{shapley1953value} are an influential approach within the removal-based explanation framework. By examining all feature subsets, they provide a nuanced view of each feature's influence and satisfy many desirable properties \citep{lundberg2017unified}. They are approximated in practice using methods like TreeSHAP and KernelSHAP \citep{lundberg2020local, covert2021improving}, but these
% current
approaches either are not applicable or do not scale to large ViTs. Recent work highlighted a connection between attention flow and Shapley values \citep{ethayarajh2021attention}, but this approach is fundamentally different from SHAP \citep{lundberg2017unified}: attention flow treats each feature's influence on the model as strictly additive, which is computationally convenient but
fails to represent feature interactions. Our work instead focuses on the original formulation \citep{lundberg2017unified} and
% makes
aims to make Shapley values based on feature removal practical for ViTs. 


==> ViT Shapley (ICLR 2023)/sections/removal.tex <==
The basic idea behind Shapley values, as well as other removal-based explanations \citep{covert2021explaining}, is to evaluate the model with partial feature information and analyze how a prediction changes. Most models need values for all the features to make predictions, so in practice we require a mechanism to represent feature removal. For example, we can set held-out image regions to zero, or we can average the prediction across randomly sampled replacement values.

With vision transformers, the options for removing features are slightly different. Recent work has demonstrated the robustness of ViTs to randomly zeroed pixel values \citep{naseer2021intriguing}, but the self-attention operation enables a more elegant approach: we can simply ignore tokens for image patches we wish to remove \citep{jain2021missingness}. We achieve this by masking attention values at each self-attention layer, or setting them to a large negative value before applying the softmax operation (see Appendix~\ref{app:masking}). This resembles causal attention masking in transformer language models like
% such as
GPT-3 \citep{brown2020language}, but we use masking for a different purpose. Alternatively, we could use a unique token value as in masked language models such as BERT \citep{devlin2018bert}, which would involve simply setting held-out tokens to the mask value.

Using this attention masking approach, we can evaluate a ViT model $f(\rvx; \eta)$ given subsets of image patches, denoted by $\rvx_\rvs$.
However, because these partial inputs represent off-manifold examples, the predictions with partial information may not behave as desired.
% However, the predictions with partial information may not behave as desired for models that were not trained with held-out tokens, because these partial inputs represent off-manifold examples.
We have two options to correct this: 1)~we can ensure that the
% original
model is trained with random masking, or 2)~we can fine-tune the model to encourage sensible behavior with missing patches.
% preserve its predictions with full images while encouraging sensible behavior with missing patches.
The first option is more direct, but it does not allow us to explain models trained without masking. For the latter option, we can create an updated model denoted by $g(\rvx_\rvs; \beta)$ that we fine-tune using the following loss,
\begin{equation}
    \min_\beta \quad \E_{p(\rvx)}\E_{p(\rvs)} 
       \Big[ \KL \big( f(\rvx; \eta) \mid\mid g(\rvx_\rvs; \beta) \big) \Big], \label{eq:surrogate}
\end{equation}
where $p(\rvs)$ is a distribution over subsets. In practice, we sample the cardinality $\rvm = \vone^\top \rvs$ from $\rvm \sim \text{Unif}(0, d)$ and then sample $\rvm$ patches uniformly at random. Intuitively, \cref{eq:surrogate} encourages $g(\rvx_\rvs; \beta)$ to preserve the original model's predictions even with missing features. We use this loss because it satisfies the desirable property that the optimal model $g(\rvx_\rvs; \beta^*)$ outputs the expected prediction given the available information \citep{covert2021explaining}, or
\begin{equation}
    g(x_s; \beta^*) = \E[f(\rvx; \eta) \mid \rvx_s = x_s].
\end{equation}
Note that this represents a best-effort prediction, because if $f(\rvx; \eta) = p(\rvy \mid \rvx)$ then we have $g(\rvx_s; \beta^*) = p(\rvy \mid \rvx_s)$. Similarly, in the case where $f(\rvx_s; \eta)$ is trained directly with random masking, the training process estimates $f(\rvx_s; \eta) \approx p(\rvy \mid \rvx_s)$ (see \Cref{app:masked_training}). We refer to the fine-tuned model $g(\rvx_\rvs; \beta)$ as a \textit{surrogate}, following the naming in prior work \citep{frye2020shapley}. Whether we use the original model or a version fine-tuned with random masking, our attention masking approach enables us to probe how individual predictions change as we remove groups of image patches.


==> figures/metrics_supplement_vitsmall_nontarget.tex <==
\begin{table}[t]
\centering
\caption{Performance metrics for non-target classes explanations
% the target class only
% with additional baselines on
with the ViT-Small architecture. Methods that fail to outperform the random baseline are shown in gray, and the best results are shown in bold (accounting for 95\% confidence intervals).
} \label{tab:metrics_supplement_vitsmall_nontarget}
\vskip 0.1in
\begin{center}
% \begin{small}
% \begin{scriptsize}
{\tablesize
    \begin{tabular}{lccc}
    \toprule
     & \multicolumn{3}{c}{ImageNette} \\
    \cmidrule(lr){2-4}
     & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
    \midrule
    Attention last & - & - & - \\
    Attention rollout & - & - & - \\\midrule
    GradCAM (LN) & 0.027 (0.002) & 0.006 (0.000) & -0.740 (0.009) \\
    GradCAM (Attn.) & \textcolor{gray}{0.008 (0.001)} & \textcolor{gray}{0.016 (0.001)} & -0.717 (0.009) \\
    IntGrad (Pixel) & 0.011 (0.001) & 0.005 (0.001) & 0.384 (0.018) \\
    IntGrad (Embed.) & 0.011 (0.001) & 0.005 (0.001) & 0.384 (0.018) \\
    Vanilla (Pixel) & 0.011 (0.001) & \textcolor{gray}{0.018 (0.001)} & -0.754 (0.009) \\
    Vanilla (Embed.) & 0.009 (0.001) & \textcolor{gray}{0.022 (0.001)} & -0.756 (0.009) \\
    SmoothGrad (Pixel) & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.027 (0.001)} & -0.756 (0.009) \\
    SmoothGrad (Embed.) & \textcolor{gray}{0.006 (0.001)} & \textcolor{gray}{0.026 (0.001)} & -0.757 (0.009) \\
    VarGrad (Pixel) & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.025 (0.001)} & -0.709 (0.009) \\
    VarGrad (Embed.) & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.024 (0.001)} & -0.723 (0.009) \\
    LRP & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.027 (0.001)} & -0.753 (0.009) \\\midrule
    Leave-one-out & 0.024 (0.002) & 0.003 (0.000) & 0.079 (0.030) \\
    RISE & 0.049 (0.004) & 0.002 (0.000) & -0.755 (0.009) \\
    \textbf{ViT Shapley} & \textbf{0.130 (0.005)} & \textbf{0.001 (0.000)} & \textbf{0.747 (0.009)} \\\midrule
    Random & \textcolor{gray}{0.007 (0.001)} & \textcolor{gray}{0.007 (0.001)} & - \\
    \bottomrule
    \end{tabular}
}
% \end{scriptsize}
% \end{small}
\end{center}
\end{table}

==> figures/metrics_supplement_vitsmall_target.tex <==
\begin{table}[t]
\centering
\caption{Performance metrics for target classes explanations
% the target class only
% with additional baselines on
with the ViT-Small architecture. Methods that fail to outperform the random baseline are shown in gray, and the best results are shown in bold (accounting for 95\% confidence intervals).
} \label{tab:metrics_supplement_vitsmall_target}
\vskip 0.1in
\begin{center}
% \begin{small}
% \begin{scriptsize}
{\tablesize
    \begin{tabular}{lccc}
    \toprule
     & \multicolumn{3}{c}{ImageNette} \\
    \cmidrule(lr){2-4}
     & Ins. ($\uparrow$) & Del. ($\downarrow$) & Faith. ($\uparrow$) \\
    \midrule
    Attention last & 0.949 (0.006) & 0.706 (0.014) & \textbf{0.781 (0.011)} \\
    Attention rollout & \textcolor{gray}{0.914 (0.007)} & 0.814 (0.013) & \textbf{0.787 (0.011)} \\\midrule
    GradCAM (LN) & \textcolor{gray}{0.908 (0.006)} & 0.898 (0.011) & 0.770 (0.010) \\
    GradCAM (Attn.) & \textcolor{gray}{0.904 (0.009)} & 0.911 (0.009) & 0.724 (0.010) \\
    IntGrad (Pixel) & 0.951 (0.006) & 0.908 (0.010) & 0.541 (0.022) \\
    IntGrad (Embed.) & 0.951 (0.006) & 0.908 (0.010) & 0.541 (0.022) \\
    Vanilla (Pixel) & \textcolor{gray}{0.905 (0.007)} & 0.830 (0.012) & \textbf{0.784 (0.010)} \\
    Vanilla (Embed.) & \textcolor{gray}{0.921 (0.007)} & 0.793 (0.013) & \textbf{0.786 (0.011)} \\
    SmoothGrad (Pixel) & \textcolor{gray}{0.943 (0.006)} & 0.744 (0.014) & \textbf{0.786 (0.011)} \\
    SmoothGrad (Embed.) & 0.946 (0.006) & 0.753 (0.014) & \textbf{0.787 (0.011)} \\
    VarGrad (Pixel) & 0.946 (0.006) & 0.766 (0.013) & 0.742 (0.010) \\
    VarGrad (Embed.) & 0.947 (0.006) & 0.774 (0.013) & 0.758 (0.010) \\
    LRP & 0.957 (0.005) & 0.695 (0.015) & \textbf{0.793 (0.010)} \\\midrule
    Leave-one-out & 0.967 (0.002) & 0.855 (0.015) & 0.044 (0.042) \\
    RISE & 0.976 (0.002) & 0.752 (0.018) & \textbf{0.787 (0.010)} \\
    \textbf{ViT Shapley} & \textbf{0.982 (0.002)} & \textbf{0.591 (0.015)} & \textbf{0.801 (0.010)} \\\midrule
    Random & \textcolor{gray}{0.933 (0.006)} & \textcolor{gray}{0.934 (0.006)} & - \\
    \bottomrule
    \end{tabular}
}
% \end{scriptsize}
% \end{small}
\end{center}
\end{table}

==> figures/qualitative_vit_shapley.tex <==
\begin{figure}[t]
    % \vspace{-.2cm}
    \centering
    \includegraphics[width=0.5\linewidth]{example-image-golden}
    \caption{
    ViT Shapley examples.
    }
    \label{fig:qualitative_vit_shapley}
\end{figure}

==> figures/roar_positional.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/roar_positional.pdf}
    \caption{
    ROAR evaluation with masked retraining, with and without positional embeddings in the retrained ViT. 
    }
    \label{fig:roar_positional}
\end{figure}
